Efficient Signature-Free Validated Agreement

Byzantine agreement enables n processes to agree on a common L-bit value, despite up to t > 0 arbitrary failures. A long line of work has been dedicated to improving the bit complexity of Byzantine agreement in synchrony. This has culminated in COOL, an error-free (deterministically secure against a computationally unbounded adversary) solution that achieves O(nL + n^2 logn) worst-case bit complexity (which is optimal for L >= n logn according to the Dolev-Reischuk lower bound). COOL satisfies strong unanimity: if all correct processes propose the same value, only that value can be decided. Strong unanimity is, however, not sufficient for today's state machine replication (SMR) and blockchain protocols. These systems value progress and require a decided value to always be valid, excluding default decisions (such as EMPTY) even in cases where there is no unanimity a priori. Validated Byzantine agreement satisfies this property (called external validity). Yet, the best error-free (or even signature-free) validated agreement solutions achieve only O(n^2L) bit complexity, a far cry from the Omega(nL + n^2) Dolev-Reishcuk lower bound. In this paper, we present two new synchronous algorithms for validated Byzantine agreement, HashExt and ErrorFreeExt, with different trade-offs. Both algorithms are (1) signature-free, (2) optimally resilient (tolerate up to t < n / 3 failures), and (3) early-stopping (terminate in O(f+1) rounds, where f <= t is the actual number of failures). On the one hand, HashExt uses only hashes and achieves O(nL + n^3 kappa) bit complexity, which is optimal for L >= n^2 kappa (where kappa is the size of a hash). On the other hand, ErrorFreeExt is error-free, using no cryptography whatsoever, and achieves O( (nL + n^2) logn ) bit complexity, which is near-optimal for any L.

==> algorithms/error_free_ext_pseudocode.tex <==
\setlength{\lineskip}{0pt}
\begin{algorithm} [hp]
\caption{\name: Pseudocode (for process $p_i$)}
\label{algorithm:recursive_early_stopping_king}
\begin{algorithmic} [1]
%\footnotesize
\fontsize{7.8pt}{7pt}\selectfont
\State \textbf{Participants:} \BlueComment{due to the recursive nature of \name, we explicitly state its set of participants}
\State \hskip2em $\mathsf{Entire} \subseteq \Pi$ with $|\mathsf{Entire}| = x$ processes 

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Set}(\mathsf{Process})$ $\mathcal{H}_1 = \{p_1, p_2, ..., p_{\lceil \frac{x}{2} \rceil}\} \setminus{\{p_\ell\}}$ \BlueComment{$p_\ell$ is a default leader, e.g., $p_\ell = p_1$}
\State \hskip2em $\mathsf{Set}(\mathsf{Process})$ $\mathcal{H}_2 = \{p_{\lceil \frac{x}{2} \rceil + 1}, ..., p_x\} \setminus{\{p_\ell\}}$
\State \hskip2em $\mathsf{Integer}$ $\beta = 7$ \BlueComment{the constant $\beta$ is explained in \Cref{subsubsection:committee_dissemination}}
\State \hskip2em \textcolor{blue}{ \(\triangleright\) the concrete values of $R_1$ and $R_2$ can be computed using the recursive equation presented in \Cref{section:name_detailed_proof}}
\State \hskip2em $\mathsf{Integer}$ $R_1 = \text{the worst-case latency complexity of \name among $\mathcal{H}_1$ with up to $|\mathcal{H}_1| / 3$ failures}$ 
\State \hskip2em $\mathsf{Integer}$ $R_2 = \text{the worst-case latency complexity of \name among $\mathcal{H}_2$ with up to $|\mathcal{H}_2| / 3$ failures}$ 

\State \hskip2em $\mathsf{Time}$ $\mathit{timeout}_1 = (R_1 + 2 + \beta)\delta$
\State \hskip2em $\mathsf{Time}$ $\mathit{timeout}_2 = (R_2 + 2 + \beta)\delta$

\medskip
\State \textbf{Uses:}
\State \hskip2em Graded consensus among $\mathsf{Entire}$, \textbf{instances} $\mathcal{GC}_{\mathit{sv}}$, $\mathcal{GC}_{\ell}$, $\mathcal{GC}_1$, $\mathcal{GC}_2$ \BlueComment{bits: $O(nL + n^2 \log n)$, rounds: $8$}
\State \hskip2em Committee broadcast $\langle \mathsf{Entire}, \{p_\ell\}, \name \rangle$, \textbf{instance} $\mathcal{CB}_{\ell}$
\State \hskip2em Committee broadcast $\langle \mathsf{Entire}, \mathcal{H}_1, \name \rangle$, \textbf{instance} $\mathcal{CB}_1$
\State \hskip2em Committee broadcast $\langle \mathsf{Entire}, \mathcal{H}_2, \name \rangle$, \textbf{instance} $\mathcal{CB}_2$
\State \hskip2em Finisher, \textbf{instances} $\mathcal{F}_{\ell}$, $\mathcal{F}_2$

\medskip
\State \textbf{Local variables:}
\State \hskip2em $\mathsf{Value}$ $v_i \gets \bot$ \BlueComment{$p_i$'s proposal}
\State \hskip2em $\mathsf{Timer}$ $\mathit{timer}_0$, $\mathit{timer}_1$, $\mathit{timer}_2$

\medskip
\State \textbf{upon} $\mathsf{propose}(\mathsf{Value} \text{ } v)$: \label{line:rec_es_propose}
\State \hskip2em $v_i \gets v$
\State \hskip2em \textbf{invoke} $\mathcal{GC}_{\mathit{sv}}.\mathsf{propose}(v_i)$ \label{line:rec_es_GCsv_propose}

\medskip
\State \textbf{upon} $\mathcal{GC}_{\mathit{sv}}.\mathsf{decide}(\mathsf{Value} \text{ } v_0, \{0, 1\} \ni g_0)$: \label{line:rec_es_GCsv_decide}
\State \hskip2em $v_i \gets v_0$ \label{line:rec_es_GCsv_update_opinion}
\State \hskip2em $\mathit{timer}_0.\mathsf{measure}\big( (2+\beta)\delta \big)$ \label{line:rec_es_GCsv_timer}
\State \hskip2em \textbf{invoke} $\mathcal{CB}_{\ell}.\mathsf{input}(v_0, g_0)$ \label{line:rec_es_EBl_propose}

\medskip
\State \textbf{upon} $\mathcal{CB}_{\ell}.\mathsf{output}(\mathsf{Value} \text{ } v')$: \label{line:rec_es_EBl_output}
\State \hskip2em \textbf{invoke} $\mathcal{GC}_\ell.\mathsf{propose}(v')$ \label{line:rec_es_GCl_propose_after_EBL}

\medskip
\State \textbf{upon} $\mathit{timer}_0$ expires: \label{line:rec_es_timer0_expires}
\State \hskip2em \textbf{invoke} $\mathcal{GC}_\ell.\mathsf{propose}(v_i)$ \label{line:rec_es_GCl_propose_after_timer}

\medskip
\State \textbf{upon} $\mathcal{GC}_\ell.\mathsf{decide}(\mathsf{Value} \text{ } v_\ell, \{0, 1\} \ni g_\ell)$: \label{line:rec_es_GCl_decide}
\State \hskip2em  $v_i \gets v_\ell$ \label{line:rec_es_GCl_update_opinion}
\State \hskip2em \textbf{invoke} $\mathcal{F}_{\ell}.\mathsf{input}(v_\ell, g_\ell)$ \label{line:rec_es_fin1_to_finish}
\State \hskip2em \textbf{wait for} $3\delta$  \label{line:rec_es_wait_1} \BlueComment{if $p_\ell$ is correct and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, without any additional steps}
\State \hskip2em \textbf{invoke} $\mathcal{GC}_1.\mathsf{propose}(v_\ell)$ \label{line:rec_es_GC1_propose}

\medskip
\State \textbf{upon} $\mathcal{F}_{\ell}.\mathsf{output}(\mathsf{Value} \text{ } v)$: \label{line:rec_es_fin1_finish}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_first_finisher}\BlueComment{will be triggered after $O(\delta)$ time if $p_\ell$ is correct and $f<n/3$}
\State \hskip2em \textbf{wait for} $2\delta$, and \textbf{stop executing} (the current instance of) \name \label{line:rec_es_halt1}


\medskip
\State \textbf{upon} $\mathcal{GC}_1.\mathsf{decide}(\mathsf{Value} \text{ } v_1, \{0, 1\} \ni g_1)$: \label{line:rec_es_GC1_decide}
\State \hskip2em  $v_i \gets v_1$: \label{line:rec_es_GC1_update_opinion}

\State \hskip2em \textbf{invoke} $\mathit{timer}_1.\mathsf{measure}(\mathit{timeout}_1)$ \label{line:rec_es_timeout1_measure}
\State \hskip2em \textbf{invoke} $\mathcal{CB}_{1}.\mathsf{input}(v_1, g_1)$ \label{line:rec_es_EB1_propose}

\medskip

\State \textbf{upon} $\mathcal{CB}_{1}.\mathsf{output}(\mathsf{Value} \text{ } v')$: \label{line:rec_es_EB1_output}
\State \hskip2em \textbf{invoke} $\mathcal{GC}_2.\mathsf{propose}(v')$ \label{line:rec_es_GC2_propose_after_EB}

\medskip
\State \textbf{upon} $\mathit{timer}_1$ expires: \label{line:rec_es_timer1_expires}
\State \hskip2em \textbf{invoke} $\mathcal{GC}_2.\mathsf{propose}(v_i)$ \label{line:rec_es_GC2_propose_after_timer}

\medskip
\State \textbf{upon} $\mathcal{GC}_2.\mathsf{decide}(\mathsf{Value} \text{ } v_2, \{0, 1\} \ni g_2)$: \label{line:rec_es_GC2_decide}
\State \hskip2em  $v_i \gets v_2$ \label{line:rec_es_GC2_update_opinion}
\State \hskip2em \textbf{invoke} $\mathcal{F}_2.\mathsf{input}(v_2, g_2)$ \label{line:rec_es_fin2_to_finish}
\State \hskip2em \textbf{wait for} $3\delta$  \label{line:rec_es_wait2} \BlueComment{if $\mathcal{H}_1$ is healthy and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}, without additional step}
\State \hskip2em \textbf{invoke} $\mathit{timer}_2.\mathsf{measure}(\mathit{timeout}_2)$ \label{line:rec_es_timeout2_measure}
\State \hskip2em \textbf{invoke} $\mathcal{CB}_{2}.\mathsf{input}(v_2, g_2)$ \label{line:rec_es_EB2_input}

\medskip
\State \textbf{upon} $\mathcal{F}_2.\mathsf{output}(v)$: \label{line:rec_es_fin2_finish}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_second_finisher}\BlueComment{will be triggered after $O(f\delta )$ time if the first half is healthy, but not $p_1$}
\State \hskip2em \textbf{wait for} $2\delta$, and \textbf{stop executing} (the current instance of)  \name \label{line:rec_es_halt2}

\medskip
\State \textbf{upon} $\mathcal{CB}_{2}.\mathsf{output}(v')$: \label{line:rec_es_EB2_output}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v')$, \textbf{wait for} $2\delta$, and \textbf{stop executing} (the current instance of)  \name \label{line:rec_es_decide_after_EB2}

\medskip
\State \textbf{upon} $\mathit{timer}_2.\mathsf{expires}$: \label{line:rec_es_timer2_expires} 
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v_i)$, \textbf{wait for} $2\delta$, and \textbf{stop executing} (the current instance of)  \name \label{line:rec_es_decide_after_timer2}

\end{algorithmic}
\end{algorithm}

==> sections/committee_dissemination_implementation_proof.tex <==
\section{Committee Dissemination: Implementation \& Proof} \label{section:dissemination}

In this section, we focus on committee dissemination, the second building block of \name.
Concretely, we introduce its implementation (\Cref{subsection:committee_dissemination_implementation}) and proof of correctness and complexity (\Cref{subsection:committee_dissemination_proof}).

\subsection{Implementation} \label{subsection:committee_dissemination_implementation}

Our implementation of the committee dissemination primitive is presented in \Cref{algorithm:committee_dissemination}.

\begin{algorithm} [h]
\caption{Committee dissemination: Pseudocode (for process $p_i$)}
\label{algorithm:committee_dissemination}
\begin{algorithmic} [1]
\footnotesize

\State Let $v^{\star}$ denote $p_i$'s input.

\medskip
\State \textbf{Round 1:} \BlueComment{executed only if $p_i \in \mathsf{Committee}$}
\State \hskip2em Let $[m_1, m_2, ..., m_{x'}] \gets \mathsf{RSEnc}(v^{\star}, x', y' + 1)$ \BlueComment{$y'$ denotes the greatest integer such that $y' < \frac{x'}{3}$}
\State \hskip2em \textbf{broadcast} $\langle \textsc{reconstruct}, m_i \rangle$ to every process $p_j \in \mathsf{Entire}$

\medskip
\State \textbf{Round 2:} \BlueComment{executed always (i.e., if $p_i \in \mathsf{Entire}$)}
\State \hskip2em Let $\mathit{rec}$ denote the number of RS symbols received via \textsc{reconstruct} messages from committee processes \label{line:received_rs_symbols}
\State \hskip2em \textbf{if} $\mathit{rec} \geq x' - y'$: \label{line:received_rs_symbols_check}
\State \hskip4em $p_i$ obtains $\mathsf{RSDec}(y' + 1, \mathit{rec} - (x' - y'), \text{received RS symbols})$ \label{line:obtain_value}
\end{algorithmic}
\end{algorithm}

\subsection{Proof of Correctness \& Complexity} \label{subsection:committee_dissemination_proof}

Recall that $|\mathsf{Entire}| = x$ and $|\mathsf{Committee}| = x' = \frac{x}{2}$.
Moreover, let $y'$ denote the greatest integer such that $y' < \frac{x'}{3}$; recall that there are at most $y'$ faulty processes in $\mathsf{Committee}$.
Finally, let $v^{\star}$ denote the common input value of all processes in $\mathsf{Committee}$.
First, we prove liveness.

\begin{theorem} [Liveness]
\Cref{algorithm:committee_dissemination} satisfies liveness.
\end{theorem}
\begin{proof}
As there are at least $x' - y'$ correct processes in $\mathsf{Committee}$, every correct process $p_i \in \mathsf{Entire}$ receives at least $x' - y'$ RS symbols via \textsc{reconstruct} messages (line~\ref{line:received_rs_symbols}).
Hence, the check at line~\ref{line:received_rs_symbols_check} passes, and $p_i$ obtains a value (line~\ref{line:obtain_value}).
% Finally, all correct processes obtain their values simultaneously as (1) they all start simultaneously, and (2) the algorithm takes exactly 2 rounds.
\end{proof}

We next prove safety.

\begin{theorem} [Safety]
\Cref{algorithm:committee_dissemination} satisfies safety.
\end{theorem}
\begin{proof}
As there are at least $x' - y'$ correct processes in $\mathsf{Committee}$, every correct process $p_i \in \mathsf{Entire}$ receives at least $x' - y'$ correctly-encoded RS symbols of value $v^{\star}$.
Moreover, $p_i$ receives at most $\mathit{rec} - (x' - y')$ incorrectly-encoded RS symbols.
Therefore, $\mathsf{RSDec}$ correctly decodes value $v^{\star}$, which concludes the proof.
\end{proof}

Finally, we prove the complexity of \Cref{algorithm:committee_dissemination}.

\begin{theorem} [Complexity]
In \Cref{algorithm:committee_dissemination}, all correct processes in $\mathsf{Committee}$ collectively send $O\big( xL + x^2 \log(x) \big)$ bits, whereas other processes send $0$ bits.
Moreover, \Cref{algorithm:committee_dissemination} takes $2 \in O(1)$ rounds.
\end{theorem}
\begin{proof}
Every correct process in $\mathsf{Committee}$ sends an RS symbol of size $O\big( \frac{L}{x'} + \log(x') \big) \in O\big( \frac{L}{x} + \log(x) \big)$.
Therefore, all correct processes in $\mathsf{Committee}$ collectively send $x' \cdot x \cdot O\big( \frac{L}{x} + \log(x) \big) \in x^2 \cdot O\big( \frac{L}{x} + \log(x) \big) \in O\big( xL + x^2 \log(x) \big)$.
Other correct processes do not send any messages.
Lastly, the algorithm indeed takes 2 rounds to terminate.
\end{proof}

==> sections/early_stopping.tex <==
\section{Recursive Early-Stopping}

\pierre{This section  will be moved into \Cref{section:name_detailed_proof}}

In this section, we present \nameES, our validated Byzantine agreement solution that achieves early stopping, i.e., adaptive $O(f)$ latency, preserving $O(nL\log n + n^2 \log n) )$ bit complexity.
The goal is to implement the former recursive structure for early-stopping. However, this approach prevents the allocation of a fixed number of rounds for a recursive call: in a run with $O(f)$ faults, only $O(f)$ rounds can be used, even if $f=o(t)$, while the recursive call must tolerate $\Omega(t)$ faults and might run longer.
Fortunately, we can modify a basic synchronization technique for lengthy inputs to guarantee that correct processes finish sub-modules within $2\delta$ time units of one another.
With this property, a simple simulation strategy allows us to treat our protocols as if they were running in perfect synchrony (the round-based paradigm). 
To do so, a round is extended to last $3\delta$. 
Finally, by employing classic locking mechanisms, correct processes that output the maximum grade from certain graded consensus instances can express their willingness to terminate early. If at least $t+1$ of these processes do so, which occurs early either due to a correct leader $p_\ell$ or a healthy half $K_1$, then the finisher enables correct processes to early agree on a common valid value and halt within $O(\delta(f+1))$ time units.
Lastly, we initiate our protocol with a single "standard" Phase King iteration involving a single king. This prevents the protocol from running for $\Theta(\log (n))$ rounds when there are only $O(1)$ faults. Consequently, we obtain a protocol that is optimally resilient and asymptotically near-optimal in terms of its early-stopping guarantee and communication complexity.








% \subsection{balanced committee dissemination} \label{subsection:balanced_committee_dissemination_implementation}

% Our balanced implementation of the committee dissemination primitive is presented in \Cref{algorithm:balanced_committee_dissemination}.

%%%%%%%%%%%%%%%%%
%% balanced CD %%
%%%%%%%%%%%%%%%%%

% \begin{algorithm} [h]
% \caption{Committee dissemination: Pseudocode (for process $p_i$)}
% \label{algorithm:balanced_committee_dissemination}
% \begin{algorithmic} [1]
% \footnotesize

% \State Let $v^{\star}$ denote $p_i$'s input.

% \medskip
% \State \textbf{Round 1:} \BlueComment{executed only if $p_i \in \mathsf{Committee}$}
% \State \hskip2em Let $[m_1, m_2, ..., m_{n}] \gets \mathsf{RSEnc}(v^{\star}, n, t + 1)$ 
% \State \hskip2em \textbf{send} $\langle \textsc{disperse}, m_j \rangle$ to every process $p_j \in \mathsf{Entire}$

% \medskip
% \State \textbf{Round 2:} \BlueComment{executed always (i.e., if $p_i \in \mathsf{Entire}$)}
% \State \hskip2em Let $\langle \textsc{disperse}, m_j \rangle$ denote the majority message received from committee processes by the first round \label{line:bcd_received_specifi_rs_symbol}.
% \State \hskip2em \textbf{broadcast} $\langle \textsc{reconstruct}, m_i \rangle$ to every process $p_j \in \mathsf{Entire}$

% \medskip
% \State \textbf{Round 3:} \BlueComment{executed always (i.e., if $p_i \in \mathsf{Entire}$)}
% \State \hskip2em Let $m_j$ denote the RS symbol sent by process $p_j$ via a \textsc{reconstruct} message ($m_j = \bot$ if such a message has not been received)
%  \label{line:bcd_received_rs_symbols}
% \State \hskip2em $p_i$ obtains $\mathsf{RSDec}(t+1, t, \{(j,m_j) | p_j \in \mathsf{Entire}\})$ \label{line:bcd_obtain_value}
% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%
%% end balanced CD %%
%%%%%%%%%%%%%%%%%%%%%

% \subsection{$\delta$-sync balanced committee dissemination} \label{subsection:nearsync_balanced_committee_dissemination_implementation}

% The first ingredient is \Cref{algorithm:delta_sync_balanced_committee_dissemination} which implements a slightly stronger version of the committee dissemination.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% delta-sync balanced CD %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm} [h]
% \caption{$\delta$-sync Committee dissemination: Pseudocode (for process $p_i$)}
% \label{algorithm:delta_sync_balanced_committee_dissemination}
% \begin{algorithmic} [1]
% \footnotesize
% \State Let $\alpha=4$
% \State Let $v^{\star}$ denote $p_i$'s input.

% \medskip
% \State \textbf{upon} $\mathsf{disseminate}(v^{\star})$ \BlueComment{executed only if $p_i \in \mathsf{Committee}$}
% \State \hskip2em Let $[m_1, m_2, ..., m_{n}] \gets \mathsf{RSEnc}(v^{\star}, n, t + 1)$ 
% \State \hskip2em \textbf{send} $\langle \textsc{symbol}, m_j \rangle$ to every process $p_j \in \mathsf{Entire}$

% \medskip
% \State \textbf{upon} receiving $t'+1$ $\langle \textsc{symbol}, m_i \rangle$ messages: \label{line:ds_bcd_received_tpp1_rs_symbols_from_committee}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{reconstruct}, m_i \rangle$ to every process $p_j \in \mathsf{Entire}$ \label{line:ds_bcd_broadcast_reconstruct}

% \medskip
% \State \textbf{upon} receiving $2t'+1$ \textsc{symbol} messages: \label{line:ds_bcd_received_2tpp1_rs_symbols_from_committee}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{enough\_started} \rangle$ to every process $p_j \in \mathsf{Entire}$ \label{line:ds_bcd_broadcast_enough_started_from_symbols}

% \medskip
% \State \textbf{upon} receiving $t+1$ \textsc{enough\_started} messages:
% \label{line:ds_bcd_received_tp1_enough_started}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{enough\_started} \rangle$ to every process $p_j \in \mathsf{Entire}$ \label{line:ds_bcd_broadcast_enough_started_from_enough_started}

% \medskip
% \State \textbf{upon} receiving $2t+1$ $\textsc{enough\_started}$ messages: \label{line:ds_bcd_received_2tp1_enough_started}
% \State \hskip2em \textbf{wait} $\alpha \delta$ time units \label{line:ds_bcd_final_waiting_step}
% \State \hskip2em Let $m_j$ denote the RS symbol sent by process $p_j$ via a \textsc{reconstruct} message ($m_j = \bot$ if such a message has not been received)
%  \label{line:ds_bcd_received_rs_symbols}
% \State \hskip2em \textbf{trigger} $\mathsf{obtain}\big(\mathsf{RSDec}(t+1, t, \{(j,m_j) | p_j \in \mathsf{Entire}\}) \big)$ \label{line:ds_bcd_obtain_value}

% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end delta-sync balanced CD %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% proof delta-sync balanced CD %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsubsection{Proof of Correctness \& Complexity} \label{subsection:delta_sync_balanced_committee_dissemination_proof}

% We want to show that \Cref{algorithm:delta_sync_balanced_committee_dissemination} solves the same properties of the Committee Dissemination problem, even if correct processes in the committee start the protocol within $(\alpha-1)\delta$ time units from each other. Moreover, \Cref{algorithm:delta_sync_balanced_committee_dissemination} also guarantees $\delta$-Totality: if a correct process obtains a value at time $\tau$, every correct process obtains a value by time $\tau+2\delta$. We underline that this property is ensured even if (i) the committee is over-corrupted, i.e. regardless the number of faulty processes in $\mathsf{Committee}$ and (ii) even if correct processes trigger the $\mathsf{disseminate}$ request with an arbitrary amount of time from each each other.

% Recall that $|\mathsf{Entire}| = x$ and $|\mathsf{Committee}| = x' \leq x$. Moreover, let $y$ denote the greatest integer such that $y < \frac{x}{3}$; recall that there are at most $y$ faulty processes in $\mathsf{Entire}$.

% We start by proving the $\delta$-Totality property

% \begin{lemma}[$\delta$-Totality]
%     \Cref{algorithm:delta_sync_balanced_committee_dissemination} ensures $\delta$-Totality, i.e. if a correct process obtains a value at time $\tau$, every correct process obtains a value by time $\tau+2\delta$.
% \end{lemma}
% \begin{proof}[proof sketch]
%     Let $p_j$ obtains a value at time $\tau_j$. The condition line \ref{line:ds_bcd_received_2tp1_enough_started} and the waiting step line \ref{line:ds_bcd_final_waiting_step}, implies that $p_j$ received $2t+1$ $\textsc{enough\_started}$ at time $\tau_j-\alpha \delta$ from a set $Q$ of $2t+1$ processes. Let $Q'$ be the subset of correct processes in $Q$. Necessarily, $|Q'| \geq t+1$. Every correct process in $Q'$ has broadcasted a $\textsc{enough\_started}$ message by time $\tau_j-\alpha\delta$. Hence, every correct process receives $t+1$ $\textsc{enough\_started}$ messages by time $\tau_j-(\alpha-1)\delta$, and broadcasts itself such an $\textsc{enough\_started}$ message by time $\tau_j-(\alpha-1)\delta$. Thus, every correct process receives $2t+1$ $\textsc{enough\_started}$ messages by time $\tau_j - (\alpha-2)\delta$. We conclude that every correct process triggers $\mathsf{obtain}$ by time $\tau_j + 2\delta$ due to the waiting step line \ref{line:ds_bcd_final_waiting_step}. This concludes the proof.
% \end{proof}

% Now, we will prove the Safety and Liveness properties of the Committee Dissemination problem, that hold under some optimistic assumptions.
% Let $y'$ denote the greatest integer such that $y' < \frac{x'}{3}$; We assume that there are at most $y'$ faulty processes in $\mathsf{Committee}$. Moreover, we assume that if a correct process triggers $\mathsf{disseminate}$ at time $\tau$, then every correct process triggers $\mathsf{disseminate}$ by time $\tau + (\alpha-1)\delta$
% Finally, let $v^{\star}$ denote the common input value of all processes in $\mathsf{Committee}$.
% First, we prove liveness.

% \begin{theorem} [Liveness]
% \Cref{algorithm:delta_sync_balanced_committee_dissemination} satisfies the following modified liveness properties: Let $\tau$ be the time when the first correct process disseminates. Then, every correct process obtains a value by time $\tau + (4 + \alpha)\delta$.
% \end{theorem}
% \begin{proof}
% As there are at least $x' - y'$ correct processes in $\mathsf{Committee}$, every correct process $p_i \in \mathsf{Entire}$ receives at least $x' - y' = 2t'+1$ $\langle \mathsf{symbol}, m_i \rangle$ messages by time $\tau + (2+1)\delta$.
% Thus, the check at line~\ref{line:ds_bcd_received_2tpp1_rs_symbols_from_committee} passes for each process by time $\tau + 3\delta$.

% This means that every correct process eventually broadcasts an $\mathsf{enough\_started}$ message by time $\tau + 3\delta$. 
% Hence, the check at line~\ref{line:ds_bcd_received_2tp1_enough_started} passes for each correct process by time $\tau + 4\delta$, and $p_i$ obtains a value (line~\ref{line:ds_bcd_obtain_value}) by time $(\tau + (4+\alpha)\delta)$.
% \end{proof}

% We next prove safety.

% \begin{theorem} [Safety]
% \Cref{algorithm:delta_sync_balanced_committee_dissemination} satisfies safety.
% \end{theorem}
% \begin{proof}
% Let $\tau$ be the time when the first correct process disseminates. 
% As there are at most $y'$ faulty processes in $\mathsf{Committee}$, 
% no correct process broadcasts a $\mathsf{reconstruct}$ message with an incorrect symbol.
% As there are at least $x' - y'$ correct processes in $\mathsf{Committee}$, every correct process $p_i \in \mathsf{Entire}$ receives at least $x' - y' = 2t'+1$ $\langle \mathsf{symbol}, m_i \rangle$ messages by time $\tau + (2+1)\delta$.
% Thus, the check at line~\ref{line:ds_bcd_received_tpp1_rs_symbols_from_committee} passes for each process by time $\tau + 3\delta$. This means every correct process broadcasts a correct symbol by time $\tau + 3\delta$, and so  every correct process receives all the correct symbols from their corresponding correct processes by time $\tau + 4\delta$.
% Let $p_i$ and $p_j$ be two correct processes that obtain a value at time $\tau_i$ and $\tau_j$ respectively. Necessarily, $\tau \leq \mathit{min}(\tau_i, \tau_j)$. Indeed, the first $\mathsf{enough\_started}$ message sent by a correct process is sent after the reception of a $\mathsf{symbol}$ message from at least $1$ (actually $t'+1$) correct process from the committee, and thus after $\tau$. Since processes $p_i$ and $p_j$ receives all the correct symbols from their corresponding correct processes by time $\tau + 4\delta = \tau + \alpha \delta$, $p_i$ and $p_j$ obtain their respective value on top of a common set of symbols from all the correct processes. Therefore, $\mathsf{RSDec}$ correctly decodes value $v^{\star}$, which concludes the proof.
% \end{proof}

% Finally, we prove the complexity of \Cref{algorithm:delta_sync_balanced_committee_dissemination}.

% \begin{theorem} [Complexity]
% In \Cref{algorithm:delta_sync_balanced_committee_dissemination}, every correct process sends $O\big(L + x \log(x) \big)$ bits.
% \end{theorem}
% \begin{proof}
% No correct process sends more than once a message with a specific header (in $\{\mathsf{reconstruct}$ $, \mathsf{symbol},$ $ \mathsf{enough\_started}\}$) 
% A $\mathsf{symbol}$ message and a $\mathsf{reconstruct}$ message both hold $O\big(\frac{L}{x} + \log(x) \big)$ bits, due to the RS symbol.
% An $\mathsf{enough\_started}$ has a size of $O(1)$ bits.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end proof delta-sync balanced CD %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Synchronizer}\label{subsection:synchronizer}

This subsection introduces the synchronizer utilized by \nameES to guarantee that processes execute different sub-modules within $2\delta$ time units of one another.
The specification of the synchronizer is given in Module~\ref{mod:synchronizer}, and its pseudocode in \Cref{algorithm:synchronizer}.
Each correct process sends $O(n)$ bits in the proposed optimally resilient ($t < n / 3$) synchronizer.

\begin{module}
\caption{Synchronizer: Specification}
\label{mod:synchronizer_2}
\footnotesize
\begin{algorithmic}[1]

\Statex \textbf{Events:}

\Statex 
\begin{compactitem}
    \item \emph{request} $\mathsf{wish\_to\_advance}()$: a process wishes to advance.

    \item \emph{indication} $\mathsf{advance}()$: a process advances.
\end{compactitem}

\medskip 
\Statex \textbf{Notes:} 
\Statex We assume that every correct process is listening and no correct process halts unless it has previously triggered the indication $\mathsf{advance}()$.

\medskip 
\Statex \textbf{Properties:}
\Statex 
\begin{compactitem}
    \item \emph{Justification:} If a correct process triggers $\mathsf{advance}()$, then at least one correct process has triggered $\mathsf{wish\_to\_advance}()$

    \item \emph{Totality:} Let $\tau$ be the first time by which a correct process has triggered $\mathsf{advance}()$. Then, every correct process triggers $\mathsf{advance}()$ by time $\tau + 2\delta$.

    \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes have triggered $\mathsf{wish\_to\_advance}()$.
    Then, every correct process triggers $\mathsf{advance}()$ by time $\tau + \delta$.

    \item \emph{Complexity:} Each correct process sends $O(n)$ bits.
\end{compactitem}
\end{algorithmic}
\end{module}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% specification synchronizer before module %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \medskip
% \noindent \textbf{Specification.}
% The synchronizer exposes the following interface:
% \begin{compactitem}
%     \item \textbf{request} $\mathsf{wish\_to\_advance}()$: a process wishes to advance.

%     \item \textbf{indication} $\mathsf{advance}()$: a process advances.
% \end{compactitem}
% We assume that every correct process is listening and no correct process halts unless it has previously triggered the indication $\mathsf{advance}()$.

% The synchronizer satisfies the following properties:
% \begin{compactitem}
%     \item \emph{Justification:} If a correct process triggers $\mathsf{advance}()$, then at least one correct process has triggered $\mathsf{wish\_to\_advance}()$

%     \item \emph{$\delta$-Totality:} Let $\tau$ be the first time by which a correct process has triggered $\mathsf{advance}()$. Then, every correct process triggers $\mathsf{advance}()$ by time $\tau + 2\delta$.

%     \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes have triggered $\mathsf{wish\_to\_advance}()$.
%     Then, every correct process triggers $\mathsf{advance}()$ by time $\tau + \delta$.

%     \item \emph{Complexity:} Each correct process sends $O(n)$ bits.
% \end{compactitem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% specification synchronizer before module (end)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\medskip
\noindent \textbf{Implementation.}
The pseudo-code of the synchronizer is presented in \Cref{algorithm:synchronizer} and has been recognized since at least the optimal clock synchronization of Srikanth an Toueg \cite{SrikanthToueg85,Srikanth1987}.


\begin{algorithm} [h]
\caption{Synchronizer: Pseudocode (for process $p_i$)}
\label{algorithm:synchronizer_2}
\begin{algorithmic} [1]
\footnotesize

\medskip
\State \textbf{upon} $\mathsf{wish\_to\_advance}()$: 
\State \hskip2em \textbf{broadcast} $\langle \textsc{wish\_to\_advance} \rangle$ 

\medskip
\State \textbf{upon} receiving $t+1$ \textsc{wish\_to\_advance} messages:
\label{line:synchronizer_received_tp1_wish_to_advance}

\State \hskip2em \textbf{broadcast} $\langle \textsc{wish\_to\_advance} \rangle$ to every process \label{line:synchronizer_broadcast_wish_to_advance_from_wish_to_advance}

\medskip
\State \textbf{upon} receiving $2t+1$ $\textsc{wish\_to\_advance}$ messages: \label{line:synchronizer_received_2tp1_wish_to_advance}
\State \hskip2em \textbf{trigger} $\mathsf{advance}()$
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\Cref{algorithm:synchronizer} implements the Synchronizer specified in \Cref{mod:synchronizer}.
\end{theorem}
\begin{proof}
    \begin{compactitem}
        \item Justification: Assume a correct process triggers $\mathsf{advance}()$. 
        Necessarily, it received a $\textsc{wish\_to\_advance}$ message. Let $p_j$ be the first correct process that has sent a $\textsc{wish\_to\_advance}$ message. Process $p_j$ has triggered $\textsc{advance}()$.
        \item Liveness: Assume every correct process triggers $\textsc{advance}()$ by time $\tau$. Then every correct process broadcasts a $\textsc{wish\_to\_advance}$ message by time $\tau$. Hence, every correct process receives $n-t$ $\textsc{wish\_to\_advance}$ message by time $\tau+\delta$. 
        \item Totality: 
          Let $p_j$ trigger $\textsc{advance}()$ at time $\tau_j$. This implies that $p_j$ received $2t+1$ $\textsc{wish\_to\_advance}$ at time $\tau_j$ from a set $Q$ of $2t+1$ processes. Let $Q'$ be the subset of correct processes in $Q$. Necessarily, $|Q'| \geq t+1$. Every correct process in $Q'$ has broadcasted a $\textsc{wish\_to\_advance}$ message by time $\tau_j$. Hence, every correct process receives $t+1$ $\textsc{wish\_to\_advance}$ messages by time $\tau_j+\delta$, and broadcasts itself such an $\textsc{wish\_to\_advance}$ message by time $\tau_j+\delta$. Thus, every correct process receives $2t+1$ $\textsc{wish\_to\_advance}$ messages by time $\tau_j +2\delta$. 

        \item Complexity: Every correct process broadcast at most one $\textsc{wish\_to\_advance}$ message.
    \end{compactitem}
\end{proof}



%%%%%%%%%%%%
\subsection{Desynchronized Committee Dissemination}

We use the simple synchronizer to implement a slightly stronger version of the committee dissemination problem, whose specification is presented in \Cref{mod:committee_dissemination_alterative}. The strengthening is (1) Safety and Liveness tolerate a ``desynchronization''  of up to $2\delta$ time units, and (2) Totality is always ensured, regardless the healthiness of the committee. The first feature is natural, since the early-stopping recursive framework inevitably leads to such a ``desynchronization''. The Totality property is essential to maintain a certain form of synchronicity, despite the execution of unhealthy halves. 

\begin{module}[h]
\caption{Robust committee dissemination $\langle \mathsf{Committee}, \mathsf{Entire} \rangle$}
\label{mod:committee_dissemination_alterative_2}
\footnotesize
\begin{algorithmic}[1]

\Statex \textbf{Participants:} \BlueComment{Typically, $|\mathsf{Committee}| \approx |\mathsf{Entire}|/2$}
\begin{compactitem}
    \item $\mathsf{Entire} \subseteq \Pi$ \BlueComment{The set of value-obtaining processes}
    \item $\mathsf{Committee} \subseteq \mathsf{Entire}$ \BlueComment{The subset of value-disseminating processes.}
\end{compactitem}
\medskip
\Statex \textbf{Events:}
\begin{compactitem}
    \item \emph{request} $\mathsf{disseminate}(v \in \mathsf{Value})$: a process $p_i \in \mathsf{Committee}$ disseminates value $v$.
    % ; a correct process $p_i$ invokes this request if and only if $p_i \in \mathsf{Committee}$.
    \item \emph{indication} $\mathsf{obtain}(v' \in \mathsf{Value})$: a process $p_i \in \mathsf{Entire}$ obtains value $v'$.
    % ; every process $p_i \in \mathsf{Entire}$ (i.e., even non-committee processes) can receive this indication.
\end{compactitem}

% \medskip 
% \Statex \textbf{Assumed behavior:}
% \begin{compactitem}
%     \item All correct processes in $\mathsf{Committee}$ disseminate the same value $v^{\star}$ (once each), and do so in the same round.
%     \item The number of faulty processes in $\mathsf{Committee}$ is less than $|\mathsf{Committee}| / 3$.
% \end{compactitem}

\medskip 
\Statex \textbf{Properties:}

% \smallskip
\begin{compactitem}
    \item \emph{Totality:} If a correct process obtains a value at time $\tau$, every correct process obtains a value by time $\tau+2\delta$.

    \item \emph{Optimistic Safety \& Liveness:} Assume all correct processes in $\mathsf{Committee}$ disseminate the same value $v^{\star}$ (once each), and do so within $2\delta$ time units of one another. Assume, the number of faulty processes in $\mathsf{Committee}$ is less than $|\mathsf{Committee}| / 3$. Then, the following properties are ensured:

    \begin{compactitem}
    
    \item \emph{Safety:} If a correct process $p_i \in \mathsf{Entire}$ obtains a value $v$, then $v = v^{\star}$.
    \item \emph{Liveness:} All correct processes in $\mathsf{Entire}$ obtain a value.
    % \item \emph{$\delta$-Timeliness:} TODO
    \item \emph{Complexity:} Each correct process sends $O(L + x\log(x))$ bits, where $x = |\mathsf{Committee}|$.
    \end{compactitem}
    
\end{compactitem}
\end{algorithmic}
\end{module}

\medskip
\noindent \textbf{Implementation.}
The pseudo-code of the robust committee dissemination is presented in \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative}. The implementation is relatively standard. We can remark that (1) processes trigger the $\mathsf{obtain}$ indication, only after having triggered $\mathsf{advance}$ from the underlying synchronizer, thus ensuring Totality in any situation, and (2) processes wait $O(\delta)$ time units before reconstructing the disseminated value, thus guaranteeing that all the correct symbols are received in the reconstruction.

\begin{algorithm} [h]
\caption{Robust Committee dissemination (alternative): Pseudocode (for process $p_i$)}
\label{algorithm:delta_sync_balanced_committee_dissemination_alternative_21}
\begin{algorithmic} [1]
\footnotesize
\State Let $\alpha=3$
\State Let $v^{\star}$ denote $p_i$'s input.
\State Let $v^{out}$ denote $p_i$'s output, initially $v^{out} = \bot$.

\medskip
    \State \textbf{Uses:}
    \State Synchronizer, \textbf{instance} $\mathcal{S}$ 
    %\State Timer, \textbf{instance} $\mathit{timer}$ 

\medskip
\State \textbf{upon} $\mathsf{disseminate}(v^{\star})$ \BlueComment{executed only if $p_i \in \mathsf{Committee}$}
\State \hskip2em Let $[m_1, m_2, ..., m_{n}] \gets \mathsf{RSEnc}(v^{\star}, n, t + 1)$ 
\State \hskip2em \textbf{send} $\langle \textsc{disperse}, m_j \rangle$ to every process $p_j \in \mathsf{Entire}$

\medskip
\State \textbf{upon} receiving $t'+1$ $\langle \textsc{disperse}, m_i \rangle$ messages: \label{line:ds_bcda_received_tpp1_rs_symbols_from_committee}
\State \hskip2em \textbf{broadcast} $\langle \textsc{reconstruct}, m_i \rangle$ to every process $p_j \in \mathsf{Entire}$ \label{line:ds_bcda_broadcast_reconstruct}

\medskip
\State \textbf{upon} receiving $2t+1$ $\textsc{reconstruct}$ messages: \label{line:ds_bcda_received_2tp1_reconstruct}
\State \hskip2em \textbf{wait} $\alpha \delta$ time units \label{line:ds_bcda_final_waiting_step}
\State \hskip2em Let $m_j$ denote the RS symbol sent by process $p_j$ via a \textsc{reconstruct} message ($m_j = \bot$ if such a message has not been received)
 \label{line:ds_bcda_received_rs_symbols}
\State \hskip2em  $v^{\mathit{out}} \gets \mathsf{RSDec}(t+1, t, \{(j,m_j) | p_j \in \mathsf{Entire}\}) \big)$ \label{line:ds_bcda_obtain_value}

\State \hskip2em \textbf{trigger} $\mathcal{S}.\mathsf{wish\_to\_advance}()$

\medskip
\State \textbf{upon} $\mathcal{S}.\mathsf{advance}()$:
\State \hskip2em \textbf{trigger} $\mathsf{obtain}(v^{\mathit{out}})$

\end{algorithmic}
\end{algorithm}

\paragraph*{Proof of Correctness \& Complexity} \label{subsection:delta_sync_balanced_committee_dissemination_alternative_proof}

We want to show that \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative} solves the same properties of the Committee Dissemination problem, even if correct processes in the committee start the protocol within $(\alpha-1)\delta$ time units from each other. Moreover, \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative} also guarantees $\delta$-Totality: if a correct process obtains a value at time $\tau$, every correct process obtains a value by time $\tau+2\delta$. We underline that this property is ensured even if (i) the committee is over-corrupted, i.e. regardless the number of faulty processes in $\mathsf{Committee}$ and (ii) even if correct processes trigger the $\mathsf{disseminate}$ request with an arbitrary amount of time from each each other.

Recall that $|\mathsf{Entire}| = x$ and $|\mathsf{Committee}| = x' \leq x$. Moreover, let $y$ denote the greatest integer such that $y < \frac{x}{3}$; recall that there are at most $y$ faulty processes in $\mathsf{Entire}$.

We start by proving the Totality property

\begin{lemma}[Totality]
    \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative} ensures Totality, i.e. if a correct process obtains a value at time $\tau$, every correct process obtains a value by time $\tau+2\delta$.
\end{lemma}
\begin{proof}
    Let $p_j$ obtains a value at time $\tau_j$. Necessarily, $p_j$ triggers $\mathcal{S}.\mathsf{advance}()$ at time $\tau_j$. By $\mathcal{S}$'s totality, every correct process triggers $\mathcal{S}.\mathsf{advance}()$ by time $\tau_j+2\delta$, and thus obtains a value by time $\tau_j+2\delta$.
\end{proof}

Now, we will prove the Safety and Liveness properties of the Committee Dissemination problem, that hold under some optimistic assumptions.
Let $y'$ denote the greatest integer such that $y' < \frac{x'}{3}$; We assume that there are at most $y'$ faulty processes in $\mathsf{Committee}$. Moreover, we assume that if a correct process triggers $\mathsf{disseminate}$ at time $\tau$, then every correct process triggers $\mathsf{disseminate}$ by time $\tau + (\alpha-1)\delta$
Finally, let $v^{\star}$ denote the common input value of all processes in $\mathsf{Committee}$.

First, we prove liveness.

\begin{lemma} [Liveness]
\Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative} satisfies the following modified liveness properties: Let $\tau$ be the time when the first correct process disseminates. Then, every correct process obtains a value by time $\tau + (5 + \alpha)\delta$.
\end{lemma}
\begin{proof}
As there are at least $x' - y'$ correct processes in $\mathsf{Committee}$, every correct process $p_i \in \mathsf{Entire}$ receives at least $x' - y' = 2t'+1$ $\langle \mathsf{Disperse}, m_i \rangle$ messages by time $\tau + (2+1)\delta$.
Thus, the check at line~\ref{line:ds_bcda_received_tpp1_rs_symbols_from_committee} passes for each process by time $\tau + 3\delta$.
This means that every correct process eventually broadcasts a $\mathsf{reconstruct}$ message by time $\tau + 3\delta$. %both a 
Hence, the check at line~\ref{line:ds_bcda_received_2tp1_reconstruct} passes for each correct process by time $\tau + 4\delta$, and each correct process triggers $\mathcal{S}.\mathsf{wish\_to\_advance}()$ by time $\tau + (\alpha+4)\delta$. By $\mathcal{S}$'s liveness, each correct process obtains a value by time $\tau + (\alpha+5)\delta$.
\end{proof}

We next prove safety.

\begin{lemma} [Safety]
\Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative} satisfies safety.
\end{lemma}
\begin{proof}
Let $p_i$ be the first correct process that obtains a value, which does so at time $\tau^o_i$.
Let $p_j$ be another correct process that obtains a value at time $\tau^o_j \geq \tau^o_j$.
By $\mathcal{S}$'s obligation, some correct process $p_k$ triggered $\mathcal{S}.\mathsf{wish\_to\_advance}$ at time $\tau^w_k \leq \tau^o_i$. The waiting step implies that $p_k$ received $2t+1$ $\mathsf{reconstruct}$ messages at time $\tau^r_k = \tau^w_k-\alpha \delta$.
Hence, some correct process $p_\ell$ has received a $\mathsf{disperse}$ message from a correct process before $\tau_r^k$.
This means that processes $p_i$ and $p_j$ receives all the correct symbols from their corresponding correct processes by time $\tau_r^k + (2+1)\delta \leq \tau^o_i - \alpha \delta + 3\delta \leq \tau^o_i$. Hence, processes $p_i$ and $p_j$ obtain their respective value on top of a common set of symbols from all the correct processes. Therefore, $\mathsf{RSDec}$ correctly decodes value $v^{\star}$, which concludes the proof.
\end{proof}

Finally, we prove the complexity of \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative}.

\begin{theorem} [Complexity]
In \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative}, every correct process sends $O\big(L + x \log(x) \big)$ bits.
\end{theorem}
\begin{proof}
No correct process sends more than once a message with a specific header (in $\{\mathsf{disperse}$ $, \mathsf{reconstruct}$ $ \mathsf{wish\_to\_advance}\}$) to another process.
A $\mathsf{disperse}$ message and a $\mathsf{reconstruct}$ message both hold $O\big(\frac{L}{x} + \log(x) \big)$ bits, due to the RS symbol.
A $\mathsf{wish\_to\_advance}$ message has a size of $O(1)$ bits.
\end{proof}

\subsection{Elector Broadcast}

We combine the (early-stopping) Byzantine agreement with the committee dissemination to obtain a new primitive, called Elector-Broadcast, presented in \Cref{mod:elector_broadcast} and thus mirror the presentation of \cite{Lenzen2022}. 
The module is intended to be executed with the output of a graded consensus' instance as input. 

\begin{module}
\caption{Elector Broadcast $\langle \mathsf{Committee}, \mathsf{Entire}, \mathcal{BA}, \mathcal{CD} \rangle$: Specification}
\label{mod:elector_broadcast}
\footnotesize
\begin{algorithmic}[1]

\Statex
\Statex \textbf{Participants:} \BlueComment{Typically, $|\mathsf{Committee}| \approx |\mathsf{Entire}|/2$}
\begin{compactitem}
    \item $\mathsf{Entire} \subseteq \Pi$, $x = |\mathsf{Entire}|$ \BlueComment{The set of value-obtaining processes}
    \item $\mathsf{Committee} \subseteq \mathsf{Entire}$, $y = |\mathsf{Committee}|$  \BlueComment{The subset of value-disseminating processes.}
\end{compactitem}

\Statex
\Statex \textbf{Uses:} 
\begin{compactitem}
    \item $\mathcal{BA}$ \BlueComment{A Byzantine Agreement module shared by $\mathsf{Committee}$} 

    %\item $\mathcal{CD}$ \BlueComment{A Robust Committe Dissemination module shared by $\langle \mathsf{Committee}, \mathsf{Entire} \rangle$} 
\end{compactitem}

\Statex
\Statex \textbf{Events:}

\Statex 
\begin{compactitem}
\item \emph{request} $\mathsf{input}(v \in \mathsf{Value}, g \in \{0,1\})$: a process proposes a pair

    \item \emph{indication} $\mathsf{output}(v \in \mathsf{Value})$: a process outputs a value.

\end{compactitem}

\medskip 
\Statex \textbf{Notes:} 
\Statex We assume that every correct process input a pair containing an externally valid value, and no correct process halts unless it has previously output. Finally, we assume that if any correct process inputs $(v, 1)$ to the Elector-Broadcast, then every
correct process inputs $(v, \cdot)$.

\medskip 
\Statex \textbf{Properties:}
\Statex 
\begin{compactitem}
    \item \emph{Totality:} Let $\tau$ be the first time by which a correct process outputs a value.  Then, every correct process outputs a value by time $\tau + 2\delta$.

    \item \emph{Stability:}
    If a correct process inputs $(v,1)$, then it returns $v$.

     \item \emph{External Validity:} No correct process outputs a value which is not externally valid.

    \item \emph{Optimistic Consensus:} If (1) there are less than $y/3$ faulty processes in $\mathsf{Committee}$, and (2) correct processes in $\mathsf{Entire}$ start within $2\delta$ time units of one another, then:
    \begin{compactitem}
    
    
    \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes in $\mathsf{Committee}$ have started. Let $\mathcal{L}_{\mathcal{BC}}(y', f')$ be the worst-case latency of the underlying $\mathcal{BA}$ among $y'$ processes with $f'$ actual failures.
    Then, every correct process outputs a value by time $\tau + \mathcal{L}_{\mathcal{BA}}(x', f') + O(\delta)$. %$+ \mathcal{L}_{\mathcal{CD}}$. 

    \item \emph{Agreement:} No two correct processes $p_i$ and $p_j$ output different values  %that input $(\cdot, 0)$ output different values 

   

    \item \emph{Strong Validity:}  If every correct process proposes $(v, \cdot)$, no correct process outputs a value different from $v$. 
    \end{compactitem}
    \item \emph{Complexity:} Each correct process sends $O\big(L + x \log(x) \big) + \mathcal{B}(y',f')$ bits, where $\mathcal{B}(y')$ is the worst-case per-process bit complexity of $\mathcal{BA}$ among $y'$ processes with $f'$ faults. 
\end{compactitem}

\end{algorithmic}
\end{module}


% \medskip
% \noindent \textbf{Specification.}
% The Elector-Broadcast exposes the following interface:
% \begin{compactitem}
%     \item \textbf{request} $\mathsf{input}(v \in \mathsf{Value}, g \in \{0,1\})$: a process proposes a pair

%     \item \textbf{indication} $\mathsf{output}(v \in \mathsf{Value})$: a process outputs a value.
% \end{compactitem}
% We assume that every correct process input a pair containing an externally valid value, and no correct process halts unless it has previously output. Finally, we assume that if any correct process inputs $(v, 1)$ to the Elector-Broadcast, then every
% correct process inputs $(v, \cdot)$.

% The Elector-Broadcast satisfies the following properties:
% \begin{compactitem}
%     \item \emph{$\delta$-Totality:} Let $\tau$ be the first time by which a correct process outputs a value.  Then, every correct process outputs a value by time $\tau + 2\delta$.

%     \item \emph{Stability:}
%     If a correct process inputs $(v,1)$, then it returns $v$.

%      \item \emph{External Validity:} No correct process outputs a value which is not externally valid.

%     \item \emph{Optimistic Consensus:} If (1) there are at most $y'$ faulty processes in $\mathsf{Committee}$, and (2) correct processes in $\mathsf{Entire}$ start within $2\delta$ time units of one another, then:
%     \begin{compactitem}
    
    
%     \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes in $\mathsf{Committee}$ have started. Let $\mathcal{L}_{\mathcal{O}}(x', f')$ be the worst-case latency of the underlying object $\mathcal{O} \in \{ \mathcal{BA}, \mathcal{CD} \}$ among $x'$ processes with $f'$ actual failures.
%     Then, every correct process outputs a value by time $\tau + \mathcal{L}_{\mathcal{BA}}(x', f') + \mathcal{L}_{\mathcal{CD}}(x', f')$. 

%     \item \emph{Agreement:} No two correct processes $p_i$ and $p_j$ output different values  %that input $(\cdot, 0)$ output different values 

   

%     \item \emph{Strong Validity:}  If every correct process proposes $(v, \cdot)$, no correct process outputs a value different from $v$. 
%     \end{compactitem}
% \end{compactitem}

\medskip
\noindent \textbf{Implementation.}
The pseudo-code of the elector broadcast is presented in \Cref{algorithm:elector_broadcast}. Essentially, \Cref{algorithm:elector_broadcast} consists in a sequential composition of Byzantine agreement and committee dissemination. Importantly, the underlying Byzantine agreement is assumed to preserve synchronicity, i.e. if (1) $\mathsf{Committee}$ counts  $f'<|\mathsf{Committee}|/3$ faulty processes and (2) all correct processes in $\mathsf{Committee}$ start $\mathcal{BA}$ within $2\delta$ time units of each other, then correct processes in $\mathsf{Committee}$ output a value from $\mathcal{BA}$ within $2\delta$ time units of each other.

\begin{algorithm} [h]
\caption{Elector Broadcast $\langle \mathsf{Committee}, \mathsf{Entire}, \mathcal{BA}, \mathcal{CD} \rangle$: Pseudocode (for process $p_i$)}
\label{algorithm:elector_broadcast}
\begin{algorithmic} [1]
\footnotesize
\State Let $(v_i, g_i)$ denote $p_i$'s input

\medskip
    \State \textbf{Uses:}
        \State Byzantine Agreement among $\mathsf{Committee}$, \textbf{instance} $\mathcal{BA}$ 
    \State Committee Dissemination from $\mathsf{Committee}$ to $\mathsf{Entire}$, \textbf{instance} $\mathcal{CD}$ \BlueComment{see \Cref{mod:committee_dissemination_alterative}} %\BlueComment{see \Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative}}

\medskip
    \State \textbf{Assumption:} 
    \State If (1) $\mathsf{Committee}$ counts  $f'<|\mathsf{Committee}|/3$ faulty processes and (2) all correct processes in $\mathsf{Committee}$ start $\mathcal{BA}$ within $2\delta$ time units of each other, then correct processes in $\mathsf{Committee}$ output a value from $\mathcal{BA}$ within $2\delta$ time units of each other \label{line:elector_broadcast_BA_assumption}

\medskip
\State \textbf{if} $p_i \in \mathsf{Committee}$: 
\State \hskip2em \textbf{trigger} $\mathcal{BA}.\mathsf{propose}(v_i)$ \label{line:elector_broadcast_BA_propose}

\medskip
\State \textbf{upon} $\mathcal{BA}.\mathsf{decide}(v^d)$ \label{line:elector_broadcast_BA_decide}
\State \hskip2em \textbf{trigger} $\mathcal{CD}.\mathsf{disseminate}(v^d)$ \label{line:elector_broadcast_CD_disseminate}

\medskip
\State \textbf{upon} $\mathcal{CD}.\mathsf{obtain}(v^o)$ \label{line:elector_broadcast_CD_obtain}
\State \hskip2em \textbf{if} $g_i = 0 \wedge \mathsf{ext\_valid}(v^o)=\mathit{true}$: \label{line:elector_broadcast_check_grade_before_returning}
\State \hskip4em \textbf{return} $v^o$ \label{line:elector_broadcast_return_obtained}
\State \hskip2em \textbf{else}:
\State \hskip4em \textbf{return} $v_i$ \label{line:elector_broadcast_return_initial}

\medskip
\State \textbf{upon} $\mathcal{B}(x')$ bits have been sent through $\mathcal{BA}$: 
\State \hskip2em \textbf{halt} $\mathcal{BA}$ \BlueComment{$p_i$ knows that $\mathsf{Committee}$ is over-corrupted}

\end{algorithmic}
\end{algorithm}

\paragraph*{Proof of correctness and complexity}

\begin{theorem}
    \Cref{algorithm:elector_broadcast} implements Elector Broadcast specified in \Cref{mod:elector_broadcast}.
\end{theorem}
\begin{proof}
$\;$
    \begin{compactitem}
        \item Totality: 
         Let $\tau$ be the first time by which a correct process $p_i$ outputs a value (line \ref{line:elector_broadcast_return_obtained} or \ref{line:elector_broadcast_return_initial}). Necessarily, $p_i$ obtains a value from $\mathcal{CD}$ at time $\tau$ (line \ref{line:elector_broadcast_CD_obtain}).
        By $\delta$-Totality of $\mathcal{CD}$, every correct process obtains a value from $\mathcal{CD}$ by time $\tau + 2\delta$ (line \ref{line:elector_broadcast_CD_obtain}). Hence, every correct process outputs a value by time $\tau + 2\delta$ (line \ref{line:elector_broadcast_return_obtained} or \ref{line:elector_broadcast_return_initial}).
        \item Stability: By the check line~\ref{line:elector_broadcast_check_grade_before_returning}.
        \item External Validity: Let $p_i$ be a correct process that outputs some value $v$ (line \ref{line:elector_broadcast_return_obtained} or \ref{line:elector_broadcast_return_initial}). If $p_i$ outputs $v$ line \ref{line:elector_broadcast_return_obtained}, then $v$ is externally valid, because of the the check line~\ref{line:elector_broadcast_check_grade_before_returning}. If $p_i$ outputs $v$ line \ref{line:elector_broadcast_return_initial}, then $v$ is externally valid, because of the assumption that a correct process always inputs a pair containing an externally valid value.
        \item Optimistic Consensus: The pre-conditions of the property ensures that $\mathcal{BA}$ guarantees the properties of Byzantine agreement. Let $\tau$ be the first time by which all correct processes in Committee have started. Let $\mathcal{L}_{\mathcal{O}}(z',f')$ be the worst-case latency of the underlying object $\mathcal{O} \in \{\mathcal{BA}, \mathcal{CD}\}$ among $z'$ processes with $f'$ actual failures. Because of the termination, agreement and external validity properties of $\mathcal{BA}$, all correct processes in $\mathsf{Committee}$ output (line~\ref{line:elector_broadcast_BA_decide}) a common externally valid value $v$ by time $\tau + \mathcal{L}_{\mathcal{BA}}(y',f')$, and do so within $2\delta$ time units of one another because of the assumption stated at line~\ref{line:elector_broadcast_BA_assumption}. Hence, all correct processes in $\mathsf{Committee}$ disseminate (line~\ref{line:elector_broadcast_CD_disseminate}) a common externally valid value $v$ by time $\tau + \mathcal{L}_{\mathcal{BA}}(y',f')$ and within $2\delta$ time units of one another.
        Because of the optimistic safety \& liveness properties of $\mathcal{CD}$, all correct processes in $\mathsf{Entire}$ obtain (line~\ref{line:elector_broadcast_CD_obtain}) the common externally valid value $v$ by time $\tau + \mathcal{L}_{\mathcal{BA}}(y',f') + \mathcal{L}_{\mathcal{CD}}$ and within $2\delta$ time units of one another, due to the $\mathcal{CD}$'s totality. Hence, all correct processes in $\mathsf{Entire}$ output some value (line~\ref{line:elector_broadcast_return_obtained} or line~\ref{line:elector_broadcast_return_initial}) by time $\tau + \mathcal{L}_{\mathcal{BA}}(y',f') + \mathcal{L}_{\mathcal{CD}}$ and within $2\delta$ time units of one another. This means that liveness is ensured. Assume no correct process has inputted $(\cdot, 1)$. Then, all correct processes output the externally valid value $v$ line~\ref{line:elector_broadcast_return_obtained} due to the check line~\ref{line:elector_broadcast_check_grade_before_returning}. Assume some correct process $p_i$ has inputted $(v_i, 1)$. In this case, we assumed that that every correct process inputs $(v_i, \cdot)$. Thus, by strong validity of $\mathcal{BA}$, $v=v_i$. Hence, all correct processes output the externally valid value $v=v_i$ either line~\ref{line:elector_broadcast_return_obtained} or line~\ref{line:elector_broadcast_return_initial}. This means that agreement is ensured. Finally, if all correct processes have inputted $(v', \cdot)$, then $v=v'$ due to $\mathcal{BA}$'s strong validity. Again, all correct processes output the externally valid value $v=v'$ either line~\ref{line:elector_broadcast_return_obtained} or line~\ref{line:elector_broadcast_return_initial}. This means that strong validity is ensured. 
    \end{compactitem}
\end{proof}

\begin{theorem}
In \Cref{algorithm:elector_broadcast}, a correct process sends $O\big(L + x \log(x) \big) + \mathcal{B}(y')$ bits, where $\mathcal{B}(x')$ is the worst-case per-process bit complexity of $\mathcal{BA}$ with less than $y'$ faults. 
\end{theorem}
\begin{proof}
    the term $O\big(L + x \log(x) \big)$ comes from $\mathcal{CD}$, while $\mathcal{B}(x')$ comes from the $\mathcal{BA}$ (A correct process handles a counter and halts if it exceeds $\mathcal{B}(x')$, meaning that the committee is not healthy). .
\end{proof}
 
\subsection{Finisher atop Synchronizer and Pre-existing Weak Agreement}\label{subsection:finisher_trivial}

Here, we present the Finisher (see~\Cref{mod:finisher}), allowing processes to decide and halt within $2\delta$ of one another, without waiting the worst case latency of the recursion. In practice, the Finisher will be executed after a graded consensus instance, making the task's realization trivial.

\begin{module}
\caption{Finisher: Specification}
\label{mod:finisher}
\footnotesize
\begin{algorithmic}[1]
\Statex
\Statex \textbf{Events:}

\Statex 
\begin{compactitem}
    \item \emph{request} $\mathsf{input}(v \in \mathsf{Value}, g \in \{0,1\})$: a process inputs a pair $(v, g)$.

    \item \emph{indication} $\mathsf{output}(v' \in \mathsf{Value})$: a process outputs value $v'$.
\end{compactitem}

\medskip 
\Statex \textbf{Notes:} 
\Statex 
We assume that all correct processes input a pair to the finisher within $2\delta$ time units of one another.
Moreover, we assume that no correct process halts unless it has previously output a value from the finisher.
Finally, we assume that if any correct process inputs $(v , 1)$ to the finisher, then every correct process inputs $(v , \cdot)$.  

\medskip 
\Statex \textbf{Properties:}
\Statex 
\begin{compactitem}
 \item \emph{Integrity:} If a correct process outputs a value $v$, then it has inputted $(v, \cdot)$

    \item \emph{Agreement:} No two correct processes output two different values.

    \item \emph{Justification:} If a correct process outputs a value, then there exists a correct process whose input is $(\cdot, 1)$.

    \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes have input the pair $(v^{\star}, 1)$ to \effin, for any value $v^{\star}$.
    Then, every correct process outputs $v^{\star}$ by time $\tau + \delta$.

     \item \emph{Totality:} Let $\tau$ be the first time by which a correct process has output a value from the finisher.
    Then, every correct process outputs a value by time $\tau + 2\delta$.

    \item \emph{Complexity:} Each correct process sends $O(n)$ bits.
\end{compactitem}

\end{algorithmic}
\end{module}

% \medskip
% \noindent \textbf{Specification.}
% The finisher \effin exposes the following interface:
% \begin{compactitem}
%     \item \textbf{request} $\mathsf{input}(v \in \mathsf{Value}, g \in \{0,1\})$: a process inputs a pair $(v, g)$.

%     \item \textbf{indication} $\mathsf{output}(v' \in \mathsf{Value})$: a process outputs value $v'$.
% \end{compactitem}
% We assume that all correct processes input a pair to the finisher within $2\delta$ time units of one another.
% Moreover, we assume that no correct process halts unless it has previously output a value from the finisher.
% Finally, we assume that if any correct process inputs $(v , 1)$ to the finisher, then every correct process inputs $(v , \cdot)$.  

% (As the finisher is employed in \nameES, the design of \nameES ensures that all of the aforementioned assumptions hold; see \Cref{subsection:early_stopping_pseudocode}.)

% The finisher satisfies the following properties:
% \begin{compactitem}
%     \item \emph{Integrity:} If a correct process outputs a value $v$, then it has inputted $(v, \cdot)$

%     \item \emph{Agreement:} No two correct processes output two different values.

%     \item \emph{Justification:} If a correct process outputs a value, then there exists a correct process whose input is $(\cdot, 1)$.

%     \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes have input the pair $(v^{\star}, 1)$ to \effin, for any value $v^{\star}$.
%     Then, every correct process outputs $v^{\star}$ by time $\tau + \delta$.

%      \item \emph{Totality:} Let $\tau$ be the first time by which a correct process has output a value from the finisher.
%     Then, every correct process outputs a value by time $\tau + 2\delta$.

%     \item \emph{Complexity:} Each correct process sends $O(n)$ bits.
% \end{compactitem}

\medskip
\noindent \textbf{Implementation.}
The pseudo-code of the finisher is presented in \Cref{algorithm:finisher_trivial}. 

\begin{algorithm} [h]
\caption{Trivial Finisher: Pseudocode (for process $p_i$)}
\label{algorithm:finisher_trivial}
\begin{algorithmic} [1]
\footnotesize
\State Let $(v_i, g_i)$ denote $p_i$'s input.

\medskip
    \State \textbf{Uses:}
    \State Synchronizer, \textbf{instance} $\mathcal{S}$ \BlueComment{See \Cref{mod:synchronizer}} 


\medskip
\State \textbf{if} $g_1=1$: \label{line:finisher_check}
\State \hskip2em \textbf{trigger} $\mathcal{S}.\mathsf{wish\_to\_advance}()$  \label{line:finisher_sync_wish}

\medskip
\State \textbf{upon} $\mathcal{S}.\mathsf{advance}()$ \label{line:finisher_sync_advance}
\State \hskip2em \textbf{trigger} $\mathsf{output}(v)$ \BlueComment{Wait the input if necessary} \label{line:finisher_output}


\end{algorithmic}
\end{algorithm}

\paragraph*{Proof of correctness and complexity}

\begin{theorem}
    \Cref{algorithm:finisher_trivial} implements the finisher specificied in \Cref{mod:finisher} with $O(n)$ bits sent per process.
\end{theorem}
\begin{proof}
$\;$
    \begin{compactitem}
        \item Integrity: a process necessarily output the value belonging to its input
        \item Justification: Assume a correct process outputs a value line~\ref{line:finisher_output}. Due to $\mathcal{S}$'s justification, a correct process triggered $\mathcal{S}.\mathsf{wish\_to\_advance}$ line~\ref{line:finisher_sync_wish}, which means it has inputted $(\cdot, 1)$ due to the check line~\ref{line:finisher_check}.
        \item Agreement: Due to the justification property and the assumption that says that if a correct process propose $(v,1)$, then every correct process proposes $(v, \cdot)$.
        \item Totality: Due to $\mathcal{S}$'s totality.
         \item Liveness: Due to $\mathcal{S}$'s liveness.
        \item Complexity: Due to $\mathcal{S}$'s complexity.
    \end{compactitem}
\end{proof}

%%%%%
% % %
%%%%%

% \subsection{\effin: Error-Free Finisher} \label{subsection:effin}

% Here, we present the finisher, allowing processes to decide and halt within $2\delta$ of one another, without waiting the worst case latency of the recursion. In practice, the finisher will be executed after a graded consensus instance, making the task's realization trivial.

% \medskip
% \noindent \textbf{Specification.}
% \effin exposes the following interface:
% \begin{compactitem}
%     \item \textbf{request} $\mathsf{input}(v \in \mathsf{Value}, g \in \{0,1\})$: a process inputs a pair $(v, g)$.

%     \item \textbf{indication} $\mathsf{output}(v' \in \mathsf{Value})$: a process outputs value $v'$.
% \end{compactitem}
% We assume that all correct processes input a pair to \effin within $2\delta$ time units of one another.
% Moreover, we assume that no correct process halts unless it has previously output a value from \effin.
% Finally, we assume that if any correct process inputs $(v \in \mathsf{Value}, 1)$ to \effin, then every correct process inputs $(v \in \mathsf{Value}, 1)$.  

% (As \effin is employed in \nameES, the design of \nameES ensures that all of the aforementioned assumptions hold; see \Cref{subsection:early_stopping_pseudocode}.)

% \effin satisfies the following properties:
% \begin{compactitem}
%     \item \emph{Agreement:} No two correct processes output two different values.

%     \item \emph{Liveness:} Let $\tau$ be the first time by which all correct processes have input a pair to \effin.
%     Then, every correct process outputs a value by time $\tau + \delta$.

%     \item \emph{Complexity:} Each correct process sends $O(L + n\log(n) )$ bits.
% \end{compactitem}

% \medskip
% \noindent \textbf{Implementation.}
% The pseudo-code \effin is presented in \Cref{algorithm:error_free_finisher}. 

% \begin{algorithm} [h]
% \caption{Error-free Finisher (Alternative): Pseudocode (for process $p_i$)}
% \label{algorithm:error_free_finisher}
% \begin{algorithmic} [1]
% \footnotesize
% \State Let $(v_i, g_i)$ denote $p_i$'s input.

% \medskip
% \State \textbf{if} $g_1=1$: 
% \State \hskip2em \textbf{broadcast} $\langle \mathsf{wish\_to\_finish} \rangle$ 

% \medskip
% \State \textbf{upon} receiving $t+1$ \textsc{wish\_to\_finish} messages:
% \label{line:effin_received_tp1_wish_to_finish}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{wish\_to\_finish} \rangle$ to every process \label{line:effin_broadcast_wish_to_finish_from_wish_to_finish}

% \medskip
% \State \textbf{upon} receiving $2t+1$ $\textsc{wish\_to\_finish}$ messages: \label{line:effin_received_2tp1_wish_to_finish}
% \State \hskip2em \textbf{trigger} $\mathsf{output}(v)$

% \end{algorithmic}
% \end{algorithm}








%%%%%%%%% % %%%%%%%%%%%%%%%%%

% We follow the algorithm \cite{Lenzen2022}

% \begin{algorithm} [h]
% \caption{Early-Stopping Phase King with Doubling Elector Set Size (for process $p_i$)}
% \label{algorithm:early_stopping_king}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Input:} Node $i$'s input $v_i \in \{0, 1\}^L$.
% \State \textbf{Output:} The node's decision on the consensus value.

% \medskip
%     \State \textbf{Constants:}
%     \State  $j_{\mathit{max}} = \lceil \log(n/6) \rceil$, $J = [0:j_{\mathit{max}}]$
% \medskip
%     \State \textbf{Uses:}
%     \State $\mathcal{K} = (K_0, K_2,...,K_{j_{\mathit{max}}})$ where $K_j = \{p_{\mathit{idx}_j}, ..., p_{\mathsf{max}(\mathit{idx}_{j+1}-1,n)}\}$ with $\mathit{idx}_j = 3\cdot 2^j + j - 2$ \BlueComment{$|K_j| = 3 \cdot 2^j + 1$}
%     \State non-adaptive Byzantine agreement algorithm~\ref{algorithm:root} among each subset $K \in \mathcal{K}$, \textbf{instances} $\{\mathcal{BA}_{K_j} \}_{j \in J}$ \BlueComment{ $\forall j\in J$, exchanged bits: $O\big(|K_j|L\log(|K_j|) + |K_j|^2\log(|K_j|) \big)$; rounds: $4 \in O(|K_j|)$}
%     \State Graded consensus, \textbf{instances} $\{\mathcal{GC}_j^{\mathit{val}}, \mathcal{GC}_j^{\mathit{term}} \}_{j \in J}$ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; rounds: $8 \in O(1)$}
% \State Committee dissemination, \textbf{instances} $\{\mathcal{CD}_{K_j} \}_{j \in J}$ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; rounds: $2 \in O(1)$}

% \medskip
% \State Initialize $op_i := v_i$.
% \State Initialize index of participants $ind := 1$.

% \medskip
% \For{$j \in [0:|J|]$}

%     \State  Process $p_i$ proposes $\mathit{op}_i$ to $\mathcal{GC}_j^{\mathit{val}}$. Let $(op_i, \mathit{strong}_i)$ be $p_i$'s decision from $\mathcal{GC}_j^{\mathit{val}}$. \BlueComment{Check if opinion change is valid (GC)}

%     \If{$p_i \in K_j$}
%         \State process $p_i$ proposes $op_i$ to $\mathcal{BA}_{K_j}$ among $K_j$, and let $op'_i$ denote $p_i$'s decision.
%         \State process $p_i$ disseminates $op'_i$ via $\mathcal{CD}_{K_j}$ with $K_j$ as a committee.
%     \EndIf
%     \State Let $p_i$ obtain value $op''_i$ from $\mathcal{CD}_{K_j}$.

%      \If{$\mathit{strong}_i = 0$}
%      \State $op_i = op''_i$
%     \EndIf
    
%     \State  Process $p_i$ proposes $\mathit{op}_i$ to $\mathcal{GC}_j^{\mathit{term}}$. Let $(op_i, \mathit{term}_i)$ be $p_i$'s decision from $\mathcal{GC}_j^{\mathit{term}}$. \BlueComment{Check for termination (GC)}
%         \State Broadcast $op_i$ \BlueComment{Termination broadcast}
%         \State \Return $op_i$ \BlueComment{Terminate}
%     \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%
%% succinct version %%
%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm} [h]
% \caption{Early-Stopping Phase King with Doubling Elector Set Size (for process $p_i$)}
% \label{algorithm:early_stopping_king_succint}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Input:} Node $i$'s input ${v}_i \in \{0, 1\}^{L}$.
% \State \textbf{Output:} The node's decision on the consensus value.

% \medskip
%     \State \textbf{Constants:}
%     \State  $j_{\mathit{max}} = \lceil \log(n/6) \rceil$, $J = [0:j_{\mathit{max}}]$
% \medskip
%     \State \textbf{Uses:}
%     \State $\mathcal{K} = (K_0, K_2,...,K_{j_{\mathit{max}}})$ where $K_j = \{p_{\mathit{idx}_j}, ..., p_{\mathsf{max}(\mathit{idx}_{j+1}-1,n)}\}$ with $\mathit{idx}_j = 3\cdot 2^j + j - 2$ \BlueComment{$|K_j| = 3 \cdot 2^j + 1$}
%     \State non-adaptive Byzantine agreement algorithm~\ref{algorithm:root} among each subset $K \in \mathcal{K}$, \textbf{instances} $\{\mathcal{BA}_{K_j} \}_{j \in J}$ \BlueComment{ $\forall j\in J$, exchanged bits: $O\big(|K_j|L\log(|K_j|) + |K_j|^2\log(|K_j|) \big)$; rounds: $4 \in O(|K_j|)$}
%     \State Graded consensus, \textbf{instances} $\{\mathcal{GC}_j^{\mathit{val}}, \mathcal{GC}_j^{\mathit{term}} \}_{j \in J}$ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; rounds: $8 \in O(1)$}
% \State Committee dissemination, \textbf{instances} $\{\mathcal{CD}_{K_j} \}_{j \in J}$ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; rounds: $2 \in O(1)$}

% \medskip
%     \State \textbf{Variables:}
% \State $op_i := v_i$.
% \State $j_{\mathit{halt}} := |J|+1$.

% \medskip
% \For{$j \in [0:|J|]$}
% \State  $(op_i, \mathit{strong}_i) \gets \mathcal{GC}_j^{\mathit{val}}.\mathsf{propose}(op_i)$.  \BlueComment{Check if opinion change is valid (GC)}

%     \If{$p_i \in K_j \wedge j<j_{\mathit{halt}}$}
%     \State $x_i \gets \mathcal{BA}(K_j).\mathsf{propose}(op_i)$
%         \State $\mathcal{CD}(K_j).\mathsf{disseminate}(x_i)$
%     \EndIf
%     \State $y_i \gets \mathcal{CD}(K_j)$'s output

%      \If{$\mathit{strong}_i = 0$}
%      \State $op_i = y_i$
%     \EndIf

%     \State $(op_i, \mathit{term}_i) \gets \mathcal{GC}_j^{\mathit{term}}.\mathsf{propose}(op_i)$.

%     \If{$term_i = 1$} \BlueComment{Check for termination}
%         \State $j_{\mathit{halt}} \gets \mathsf{min}(j+1, j_{\mathit{halt}})$ \BlueComment{Halt at most in the next iteration}
%         \State \textbf{decide} $op_i$ 
%         \If{$j_{\mathit{halt}} = j$}
%         \State \textbf{halt} \BlueComment{Terminate}
%             \EndIf
%     \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% \begin{lemma}
%     \Cref{algorithm:early_stopping_king_succint} solves Byzantine consensus
% \end{lemma}
% \begin{proof}[sketch]
% \begin{itemize}
%     \item Strong Validity: If all the correct processes start with the same value, the two consecutive graded consensus instances, and the fact that the output of the committee dissemination will be ignored ensure strong validity. 

%     \item Agreement: If a process decide, then no disagreement is possible because of the to graded consensus instances, and the fact that the output of the committee dissemination will be ignored

%     \item External Validity: comes from an implicit sanity check at each step.

%     \item Termination: If a correct process decides at iteration $j$, every correct process decides by iteration $j+1$. Assume no correct process decided at the beginning of iteration $j$, where $K_j$ is the first healthy committee in $\mathcal{K}$. If some correct process $p_i$ obtains $(op_i, \mathit{strong}_i=1)$ from $\mathcal{GC}_j^{\mathit{val}}$, then, by $\mathcal{GC}_j^{\mathit{val}}$'s consistency every correct process obtains $(op_i, \cdot)$ from $\mathcal{GC}_j^{\mathit{val}}$. Therefore, by $\mathcal{BA}(K_j)$'s strong validity, every correct process in $K_j$ outputs $x_i = op_i$ from $\mathcal{BA}(K_j)$. Thereupon, by $\mathcal{CD}(K_j)$'s safety, every correct process obtains $y_i = op_i$ from $\mathcal{CD}(K_j)$. Hence, the opinion of any correct process before entering $\mathcal{GC}_j^{\mathit{term}}$ is $op_i$. By $\mathcal{GC}_j^{\mathit{term}}$'s strong validity, every correct process decides $op_i$ in iteration $j$ 
%     and halt in iteration $j+1$.
    
% \end{itemize}



% \end{proof}

% \begin{lemma}
%     Correct processes decide and halt after $O(f)$ rounds in \Cref{algorithm:early_stopping_king_succint}. 
% \end{lemma}
% \begin{proof}[sketch]
%     Let $j_{\mathit{ada}} = \log(f/2)$. By iteration $j_{\mathit{ada}}$, every correct process decides 
%     and halt in the next iteration. The running time is $O \big(\sum_{j=0}^{j_{\mathit{ada}}} 2^j + 1 \big)= O(f+1)$
% \end{proof}

% \begin{lemma}
%     Any correct process sends $O(Llog(f)+nlog(f))$ bits in \Cref{algorithm:early_stopping_king_succint}, ignoring committee dissemination. 
% \end{lemma}
% \begin{proof}[sketch]
%     Let $j_{\mathit{ada}} = \log(f/2)$. By iteration $j_{\mathit{ada}}$, every correct process decides 
%     and halt in the next iteration. We ignore the committee-dissemination. The per-process bit complexity is 
    
%     $O \big( \sum_{j=0}^{j_{\mathit{ada}+1}} L\log(|K_j|) + n\log(n) \big) = O(L\cdot (1+\log(f+1))^2 + n \cdot \log(n) \cdot (1+\log(f+1)))$
%     %$O \big( \sum_{j=0}^{j_{\mathit{ada}+1}} (|K_j| \log(|K_j|)) + L + n\log(n) \big) = O(f+1)$
% \end{proof}

% \begin{lemma}
%     Any correct process that participates to $\mathcal{CD}(K_j)$ (\Cref{algorithm:committee_dissemination}) as a member of the committee $K_j$ sends $n$ messages of size $L/|K_j|$.
% \end{lemma}
% \begin{proof}
%     Trivial.
% \end{proof}

\subsection{\nameES: Recursive Early-Stopping VBA}\label{subsection:early_stopping_pseudocode}

This subsection presents \nameES (see figure~\ref{fig:early stopping recursive framework}), an error-free Byzantine agreement algorithm that achieves (1) $O\big( nL\log n + n^2 \log n \big)$ bit complexity, and (2) $O(f\delta)$ latency.
We present \nameES's pseudocode (\Cref{algorithm:recursive_early_stopping_king}) and prove its correctness and complexity.

\begin{algorithm} [hp]
\caption{\nameES among $\{p_1, ..., p_n\}$: Recursive Early-Stopping Phase King (for process $p_i$)}
\label{algorithm:recursive_early_stopping_king}
\begin{algorithmic} [1]
\footnotesize

\State \textbf{Input:} Node $i$'s input ${v}_i \in \{0, 1\}^{L}$.
\State \textbf{Output:} The node's decision on the consensus value.


\medskip
    \State \textbf{Functions:}
    \State $\mathsf{wc\_latency} : [1:\lceil n/2 \rceil ]\rightarrow \mathbb{R}$ \BlueComment{returns the worst case latency of the Recursive Early-Stopping Phase King protocol among $n' \in [1:\lceil n/2 \rceil ]$ processes}
    

\medskip
    \State \textbf{Constants:}
    \State  $\mathsf{timeout} =\mathit{max}\big(\mathsf{wc\_latency}(\lceil n/2\rceil ), \mathsf{wc\_latency}(\lfloor n/2\rfloor ) \big) + (4+\alpha)\delta$
     \State $(K_1, K_2) = (\{p_1, ..., \lceil n/2 \rceil\} \setminus \{p_\ell\}, \{\lceil n/2 \rceil+1, ... p_n\} \setminus \{p_\ell\})$
    
\medskip
    \State \textbf{Uses:}
    \State Graded consensus, \textbf{instances} $\mathcal{GC}_{\mathit{sv}}, \mathcal{GC}_\ell, \mathcal{GC}_1, \mathcal{GC}_2 $ \BlueComment{exchanged bits: $O\big( nL + n^2\log n \big)$; rounds: $8 \in O(1)$}


    
    \State Byzantine agreement~(\Cref{algorithm:recursive_early_stopping_king}) among subsets $\{p_\ell\}$, $K_1$ and $K_2$, \textbf{instances} $\{ \mathcal{BA}_{\{p_\ell\}}, \mathcal{BA}_{K_1}, \mathcal{BA}_{K_2} \}$ 

    \State Elector broadcast (\Cref{algorithm:elector_broadcast}) with $\{p_1\}$, $K_1$ and $K_2$ as committee respectively and $ \mathcal{BA}_{\{p_\ell\}}, \mathcal{BA}_{K_1}, \mathcal{BA}_{K_2} $ as underlying Byzantine agreement protocols respectively,  \textbf{instances} $ \mathcal{EB}_{\{p_\ell\}}, \mathcal{EB}_{K_1}, \mathcal{EB}_{K_2} $

 \State Finisher~(\Cref{algorithm:finisher_trivial}) \textbf{instances} $\mathcal{F}_1$, $\mathcal{F}_2$


\medskip
    \State \textbf{Variables:}
\State $op_i := v_i$.
\State $\mathit{timer}_0, \mathit{timer}_1, \mathit{timer}_2$.

\medskip
\State \textbf{upon} $\mathsf{propose}(op_i)$: \label{line:rec_es_propose}
\State \hskip2em $\mathcal{GC}_{sv}.\mathsf{propose}(op_i)$ \label{line:rec_es_GCsv_propose}

\medskip
\State \textbf{upon} $\mathcal{GC}_{sv}.\mathsf{decide}(v_0, g_0)$: \label{line:rec_es_GCsv_decide}
\State \hskip2em $op_i \gets v_0$ \label{line:rec_es_GCsv_update_opinion}
\State \hskip2em $\mathit{timer}_0.\mathsf{measure}((4+\alpha)\delta)$ \label{line:rec_es_GCsv_timer}
\State \hskip2em $\mathcal{EB}_{\{p_\ell\}}.\mathsf{propose}(v_0, g_0)$ \label{line:rec_es_EBl_propose}

\medskip
\State \textbf{upon} $\mathcal{EB}_{\{p_\ell\}}.\mathsf{output}(v')$: \label{line:rec_es_EBl_output}
\State \hskip2em $\mathcal{GC}_\ell.\mathsf{propose}(v')$ \label{line:rec_es_GCl_propose_after_EBL}

\medskip
\State \textbf{upon} $\mathit{timer}_0.\mathsf{expires}$: \label{line:rec_es_timer0_expires}
\State \hskip2em $\mathcal{GC}_\ell.\mathsf{propose}(op_i)$ \label{line:rec_es_GCl_propose_after_timer}

\medskip
\State \textbf{upon} $\mathcal{GC}_\ell.\mathsf{decide}(v_\ell, g_\ell)$: \label{line:rec_es_GCl_decide}
\State \hskip2em  $op_i \gets v_\ell$ \label{line:rec_es_GCl_update_opinion}
\State \hskip2em $\mathcal{F}_1.\mathsf{to\_finish}(v_\ell, g_\ell)$ \label{line:rec_es_fin1_to_finish}
\State \hskip2em \textbf{wait} $3\delta$  \label{line:rec_es_wait_1} \BlueComment{If $p_\ell$ is correct and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, without additional step}
\State \hskip2em $\mathcal{GC}_1.\mathsf{propose}(v_\ell)$ \label{line:rec_es_GC1_propose}

\medskip
\State \textbf{upon} $\mathcal{F}_1.\mathsf{finish}(v)$: \label{line:rec_es_fin1_finish}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_first_finisher}\BlueComment{will be triggered after $O(\delta)$ time if $p_\ell$ is correct and $f<n/3$}
\State \hskip2em \textbf{halt} the current instance \label{line:rec_es_halt1}

\medskip
\State \textbf{upon} $\mathcal{GC}_1.\mathsf{decide}(v_1, g_1)$: \label{line:rec_es_GC1_decide}
\State \hskip2em  $op_i \gets v_1$: \label{line:rec_es_GC1_update_opinion}

\State \hskip2em $\mathit{timer}_1.\mathsf{measure}(\mathsf{timeout})$ \label{line:rec_es_timeout1_measure}
\State \hskip2em $\mathcal{EB}_{K_1}.\mathsf{propose}(v_1, g_1)$ \label{line:rec_es_EB1_propose}

\medskip

\State \textbf{upon} $\mathcal{EB}_{K_1}.\mathsf{output}(v')$: \label{line:rec_es_EB1_output}
\State \hskip2em $\mathcal{GC}_2.\mathsf{propose}(v')$ \label{line:rec_es_GC2_propose_after_EB}

\medskip
\State \textbf{upon} $\mathit{timer}_1.\mathsf{expires}$: \label{line:rec_es_timer1_expires}
\State \hskip2em $\mathcal{GC}_2.\mathsf{propose}(op_i)$ \label{line:rec_es_GC2_propose_after_timer}

\medskip
\State \textbf{upon} $\mathcal{GC}_2.\mathsf{decide}(v_2, g_2)$: \label{line:rec_es_GC2_decide}
\State \hskip2em  $op_i \gets v_2$ \label{line:rec_es_GC2_update_opinion}
\State \hskip2em $\mathcal{F}_2.\mathsf{to\_finish}(v_2, g_2)$ \label{line:rec_es_fin2_to_finish}
\State \hskip2em \textbf{wait} $3\delta$  \label{line:rec_es_wait2} \BlueComment{If $K_1$ is healthy and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}, without additional step}
\State \hskip2em $\mathit{timer}_2.\mathsf{measure}(\mathsf{timeout})$ \label{line:rec_es_timeout2_measure}
\State \hskip2em $\mathcal{EB}_{K_2}.\mathsf{input}(v_2, g_2)$ \label{line:rec_es_EB2_input}

\medskip
\State \textbf{upon} $\mathcal{F}_2.\mathsf{finish}(v)$: \label{line:rec_es_fin2_finish}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_second_finisher}\BlueComment{will be triggered after $O(f\delta )$ time if the first half is healthy, but not $p_1$}
\State \hskip2em \textbf{halt} the current instance \label{line:rec_es_halt2}

\medskip
\State \textbf{upon} $\mathcal{EB}_{K_2}.\mathsf{output}(v')$: \label{line:rec_es_EB2_output}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v')$, wait $2\delta$, and \textbf{halt} \label{line:rec_es_decide_after_EB2}\BlueComment{triggered after $O(t\delta)$ time, only if $K_1$ is not healthy, i.e. $f \geq n/6$}

\medskip
\State \textbf{upon} $\mathit{timer}_2.\mathsf{expires}$: \label{line:rec_es_timer2_expires} 
\State \hskip2em \textbf{trigger} $\mathsf{decide}(op_i)$, wait $2\delta$, and \textbf{halt} \label{line:rec_es_decide_after_timer2}\BlueComment{triggered after $O(t\delta)$ time, only if $f>n/3$}

\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% recursive early stopping (old) %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm} [hp]
% \caption{\nameES among $\{p_1, ..., p_n\}$: Recursive Early-Stopping Phase King (for process $p_i$)}
% \label{algorithm:recursive_early_stopping_king}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Input:} Node $i$'s input ${v}_i \in \{0, 1\}^{L}$.
% \State \textbf{Output:} The node's decision on the consensus value.


% \medskip
%     \State \textbf{Functions:}
%     \State $\mathsf{wc\_latency} : [1:\lceil n/2 \rceil ]\rightarrow \mathbb{R}$ \BlueComment{returns the worst case latency of the Recursive Early-Stopping Phase King protocol among $n' \in [1:\lceil n/2 \rceil ]$ processes}
    

% \medskip
%     \State \textbf{Constants:}
%     \State  $\mathsf{timeout} =\mathit{max}\big(\mathsf{wc\_latency}(\lceil n/2\rceil ), \mathsf{wc\_latency}(\lfloor n/2\rfloor ) \big) + (4+\alpha)\delta$
%      \State $(K_1, K_2) = (\{p_2, ..., \lceil n/2 \rceil\}, \{\lceil n/2 \rceil+1, ... p_n\})$
    
% \medskip
%     \State \textbf{Uses:}
%     \State Graded consensus, \textbf{instances} $\mathcal{GC}_0, \mathcal{GC}_1, \mathcal{GC}_2 $ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; rounds: $8 \in O(1)$}


    
%     \State Byzantine agreement~(\Cref{algorithm:recursive_early_stopping_king}) among subsets $\{p_1\}$, $K_1$ and $K_2$, \textbf{instances} $\{ \mathcal{BA}_{\{p_1\}}, \mathcal{BA}_{K_1}, \mathcal{BA}_{K_2} \}$ 

%     \State Elector broadcast (\Cref{algorithm:elector_broadcast}) with $\{p_1\}$, $K_1$ and $K_2$ as committee respectively and $ \mathcal{BA}_{\{p_1\}}, \mathcal{BA}_{K_1}, \mathcal{BA}_{K_2} $ as underlying Byzantine agreement protocols respectively,  \textbf{instances} $ \mathcal{EB}_{\{p_1\}}, \mathcal{EB}_{K_1}, \mathcal{EB}_{K_2} $

% % \State Committee dissemination~(\Cref{algorithm:delta_sync_balanced_committee_dissemination_alternative}) with $K_1$ and $K_2$ as committee respectively, \textbf{instances} $\{\mathcal{CD}_{K_1}, \mathcal{CD}_{K_2} \}$ \BlueComment{exchanged bits: $O\big( nL + n^2\log(n) \big)$; latency: $(4 + \alpha) \delta \in O(\delta)$}
%  \State Finisher~(\Cref{algorithm:finisher_trivial}) \textbf{instances} $\mathcal{F}_1$, $\mathcal{F}_2$


% \medskip
%     \State \textbf{Variables:}
% \State $op_i := v_i$.
% \State $\mathit{timer}_0, \mathit{timer}_1, \mathit{timer}_2$.

% \medskip
% \State \textbf{upon} $\mathsf{propose}(op_i)$:
% \State \hskip2em $\mathcal{GC}_0.\mathsf{propose}(op_i)$

% \medskip
% \State \textbf{upon} $\mathcal{GC}_0.\mathsf{decide}(v_0, g_0)$:
% \State \hskip2em $op_i \gets v_0$
% \State \hskip2em $\mathit{timer}_0.\mathsf{measure}((4+\alpha)\delta)$
% \State \hskip2em $\mathcal{EB}_{\{p_1\}}.\mathsf{propose}(v_0, g_0)$

% \medskip
% \State \textbf{upon} $\mathcal{EB}_{\{p_1\}}.\mathsf{output}(v')$:
% %\State \hskip2em $op_i \gets v'$
% \State \hskip2em $\mathcal{GC}_1.\mathsf{propose}(v')$

% \medskip
% \State \textbf{upon} $\mathit{timer}_0.\mathsf{expires}$:
% \State \hskip2em $\mathcal{GC}_1.\mathsf{propose}(op_i)$

% \medskip
% \State \textbf{upon} $\mathcal{GC}_1.\mathsf{decide}(v_1, g_1)$:

% %\State \hskip2em \textbf{if} $g_1=1$:
% %\State \hskip4em  $op_i \gets v_1$:

% \State \hskip2em  $op_i \gets v_1$:
% \State \hskip2em $\mathcal{F}_1.\mathsf{to\_finish}(v_1, g_1)$ 
% \State \hskip2em \textbf{wait} $3\delta$   \BlueComment{If $p_1$ is correct and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, without additional step}

% \State \hskip2em $\mathit{timer}_1.\mathsf{measure}(\mathsf{timeout})$
% \State \hskip2em $\mathcal{EB}_{K_1}.\mathsf{propose}(v_1, g_1)$
% % \State \hskip2em \textbf{if} $p_i \in K_1$:
% % \State \hskip4em $\mathcal{BA}_{K_1}.\mathsf{propose}(op_i)$

% % \medskip
% % \State \textbf{upon} $\mathcal{BA}_{K_1}.\mathsf{decide}(v^{*})$:
% % \State \hskip2em  $\mathcal{CD}_{K_1}.\mathsf{disseminate}(v^{*})$

% \medskip
% \State \textbf{upon} $\mathcal{F}_1.\mathsf{finish}(v)$:
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_first_finisher}\BlueComment{will be triggered after $O(\delta )$ time if $p_1$ is correct and $f<n/3$}
% \State \hskip2em \textbf{halt} the current instance

% \medskip
% %\State \textbf{upon} $\mathcal{CD}_{K_1}.\mathsf{obtains}(v')$:
% \State \textbf{upon} $\mathcal{EB}_{K_1}.\mathsf{output}(v')$:
% %\State \hskip2em  \textbf{if} $g_1 = 0 \wedge \mathsf{ext\_valid}(v')$:
% % \State \hskip2em $op_i \gets v'$
% % \State \hskip2em $\mathcal{GC}_2.\mathsf{propose}(op_i)$
% \State \hskip2em $\mathcal{GC}_2.\mathsf{propose}(v')$

% \medskip
% \State \textbf{upon} $\mathit{timer}_1.\mathsf{expires}$:
% \State \hskip2em $\mathcal{GC}_2.\mathsf{propose}(op_i)$

% %%%
% \medskip
% \State \textbf{upon} $\mathcal{GC}_2.\mathsf{decide}(v_2, g_2)$:
% \State \hskip2em $\mathit{timer}_2.\mathsf{measure}(\mathsf{timeout})$
% % \State \hskip2em \textbf{if} $g_2=1$:
% % \State \hskip4em  $op_i \gets v_2$
% \State \hskip2em  $op_i \gets v_2$
% \State \hskip2em $\mathcal{F}_2.\mathsf{to\_finish}(v_2, g_2)$
% \State \hskip2em \textbf{wait} $3\delta$   \BlueComment{If $K_1$ is healthy and $f<n/3$, decision is made at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}, without additional step}
% % \State \hskip2em \textbf{if} $p_i \in K_2$:
% % \State \hskip4em $\mathcal{BA}_{K_2}.\mathsf{propose}(v_2)$
% \State \hskip2em $\mathcal{EB}_{K_2}.\mathsf{input}(v_2, g_2)$

% % \medskip
% % \State \textbf{upon} $\mathcal{BA}_{K_2}.\mathsf{decide}(v^{*})$:
% % \State \hskip2em  $\mathcal{CD}_{K_2}.\mathsf{disseminate}(v^{*})$

% \medskip
% \State \textbf{upon} $\mathcal{F}_2.\mathsf{finish}(v)$:
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(v)$ \label{line:recursive_early_stopping_decide_after_second_finisher}\BlueComment{will be triggered after $O(f\delta )$ time if the first half is healthy, but not $p_1$}
% \State \hskip2em \textbf{halt} the current instance

% \medskip
% %\State \textbf{upon} $\mathcal{CD}_{K_2}.\mathsf{obtains}(v')$:
% \State \textbf{upon} $\mathcal{EB}_{K_2}.\mathsf{output}(v')$:
% %\State \hskip2em  \textbf{if} $g_2 = 0 \wedge \mathsf{ext\_valid}(v')$:
% %\State \hskip2em $op_i \gets v'$
% %\State \hskip2em \textbf{trigger} $\mathsf{decide}(op_i)$
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(v')$ \BlueComment{triggered after $O(t\delta)$ time, only if $K_1$ is not healthy, i.e. $f \geq n/6$}

% \medskip
% \State \textbf{upon} $\mathit{timer}_2.\mathsf{expires}$: 
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(op_i)$ \BlueComment{triggered after $O(t\delta)$ time, only if $f>n/3$}



% \end{algorithmic}
% \end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% end recursive early stopping (old) %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph*{Proof of Correctness and Complexity}

As \nameES is a recursive algorithm, we start by showing that \name with $n = 1$ is correct.

\begin{theorem} [\nameES is correct if $n = 1$]
If $n = 1$, \nameES is correct.
\end{theorem}
\begin{proof}
Let $p_i$ be the only correct process. 
Strong validity follows from the fact that $p_i$ decides its own proposal.
Due to the assumption that $p_i$'s proposal is valid, external validity is satisfied.
Termination, integrity, and agreement are trivially satisfied.
\end{proof}


In the remainder of the proof, we establish the correctness of the \nameES algorithm among 
$n$ processes, assuming that (1) the \nameES algorithm functions correctly among $\lceil \frac{n}{2} \rceil$ and $\lfloor \frac{n}{2} \rfloor$ , provided that less than one-third of these processes are faulty.
%\mv{This sentence is confusing. I put an alternative one commented below. Check if it matches.}
% In the rest of the proof, we prove that \nameES among $n$ processes is correct assuming that (1) \name operating among $\lceil \frac{n}{2} \rceil$ or $\lfloor \frac{n}{2} \rfloor$ processes is correct when less than one-third of processes ($\lceil \frac{n}{6} \rceil$ or $\lfloor \frac{n}{6} \rfloor$ respectively) are faulty.
We start by showing that every module works according to its specification.
%$\mathcal{GC}_0$, $\mathcal{GC}_1$, $\mathcal{GC}_2$, $\mathcal{EB}_{\{p_1\}}$, $\mathcal{EB}_{K_1}$, $\mathcal{EB}_{K_2}$, $\mathcal{F}_{1}$, and $\mathcal{F}_{2}$

%%%%%%%%
%% %% %%
\begin{lemma}
\label{lemma:res_spec_assumption}
Assume that all correct processes propose a value within $2\delta$ time of each other. Then, all correct processes decide on an externally-valid value within $2\delta$ time of each other. Moreover, every correct process proposes only valid values to $\mathcal{GC}_{sv}$, $\mathcal{GC}_{0}$, $\mathcal{GC}_1$, $\mathcal{GC}_2$, $\mathcal{EB}_{\{p_\ell\}}$, $\mathcal{EB}_{K_1}$, $\mathcal{EB}_{K_2}$, $\mathcal{F}_{1}$, and $\mathcal{F}_{2}$ within $2\delta$ time of one another. Furthermore, if a correct process proposes $(v,1)$ to some object in $\{ \mathcal{EB}_{\{p_\ell\}}, \mathcal{EB}_{K_1}, \mathcal{EB}_{K_2}, \mathcal{F}_{1}, \mathcal{F}_{2}\}$, then every correct process proposes $(v,\cdot)$ to this object.
\end{lemma}
\begin{proof}
Consider any pair of correct processes $(p_i, p_j)$.
\begin{compactitem}
    \item $\mathcal{GC}_{sv}$: Process $p_i$ proposes a valid value to $\mathcal{GC}_{sv}$ (line~\ref{line:rec_es_GCsv_propose}) because (1) $p_i$ forwards its proposal to \nameES to $\mathcal{GC}_{sv}$, and (2) $p_i$'s proposal to \nameES is valid (due to the assumption). All correct processes propose a value within $2\delta$ time since they immediately forward their proposal proposed within $2\delta$ time of one another.

    \item $\mathcal{EB}_{\{p_\ell\}}$: Correct processes propose valid values to $\mathcal{EB}_{\{p_\ell\}}$ (line~\ref{line:rec_es_EBl_propose}) due to $\mathcal{GC}_{sv}$'s external validity. Moreover, the simulation (each $\mathcal{GC}_{sv}$'s round lasts $3\delta$) implies they do so within $2\delta$ time of each other. Upon $\mathcal{GC}_{sv}$'s termination (line~\ref{line:rec_es_GCsv_decide}), they immediately trigger their respective timer (line~\ref{line:rec_es_GCsv_timer}) that will expire within $2\delta$ time of each other. Let $\tau^{0}_e$ denote the time at which the first timer expires (line~\ref{line:rec_es_timer0_expires}). If $p_j$ proposes $(v, 1)$ to $\mathcal{EB}_{\{p_\ell\}}$ (line~\ref{line:rec_es_EBl_propose}), then $p_i$ proposes $(v, \cdot)$ to $\mathcal{EB}_{\{p_\ell\}}$ (line~\ref{line:rec_es_EBl_propose}), due to $\mathcal{GC}_{sv}$'s consistency.

    \item $\mathcal{GC}_\ell$: Correct processes propose valid values to $\mathcal{GC}_\ell$ as any correct process proposes either (line~\ref{line:rec_es_GCl_propose_after_EBL}) the output of $\mathcal{EB}_{\{p_\ell\}}$, which is externally valid due to $\mathcal{EB}_{\{p_\ell\}}$'s external validity or (line~\ref{line:rec_es_GCl_propose_after_timer}) $\mathcal{GC}_{sv}$'s output which is valid due to $\mathcal{GC}_{sv}$'s external validity. They do so within $2\delta$ time of each other. Indeed, if some correct process proposes a value (line~\ref{line:rec_es_GCl_propose_after_timer}) because of the timer expiration, it does so between $\tau^{0}_e$ and $\tau^{0}_e + 2\delta$. Assume a correct process proposes (line~\ref{line:rec_es_GCl_propose_after_EBL}) a value coming from $\mathcal{EB}_{\{p_\ell\}}$. It necessarily proposes it before $\tau^{0}_e + 2\delta$. Let $\tau' \leq \tau^{0}_e + 2\delta$ be the time at which the first correct proposes a value (line~\ref{line:rec_es_GCl_propose_after_EBL}) coming from $\mathcal{EB}_{\{p_\ell\}}$. By $\mathcal{EB}_{\{p_\ell\}}$'s totality, every correct process proposes a value to $\mathcal{GC}_\ell$ (line~\ref{line:rec_es_GCl_propose_after_EBL} or line~\ref{line:rec_es_GCl_propose_after_timer}) between $\mathsf{min}(\tau^{0}_e, \tau')$ and $\mathsf{min}(\tau^{0}_e, \tau') + 2 \delta$.

    \item $\mathcal{F}_1$: Correct processes propose (line~\ref{line:rec_es_fin1_finish}) valid values to $\mathcal{F}_1$ within $2\delta$ time of each other because of $\mathcal{GC}_{\ell}$'s external validity. If $p_j$ proposes $(v, 1)$ to $\mathcal{F}_{1}$, then $p_i$ proposes $(v, \cdot)$ to $\mathcal{F}_{1}$, due to $\mathcal{GC}_{\ell}$'s consistency.

    \item $\mathcal{GC}_1$: Correct processes propose (line~\ref{line:rec_es_GC1_propose}) valid values to $\mathcal{GC}_1$ within $2\delta$ time of each other because of $\mathcal{GC}_{\ell}$'s external validity. If $p_j$ proposes $(v, 1)$ to $\mathcal{GC}_{1}$, then $p_i$ proposes $(v, \cdot)$ to $\mathcal{GC}_{1}$, due to $\mathcal{GC}_{\ell}$'s consistency.

    \item $\mathcal{EB}_{K_1}$: Process $p_i$ proposes (line~\ref{line:rec_es_EB1_propose}) a valid value to $\mathcal{EB}_{K_1}$ because of $\mathcal{GC}_1$'s external validity. The simulation (each $\mathcal{GC}_{1}$'s round lasts $3\delta$) implies they do so within $2\delta$ time of each other. Upon $\mathcal{GC}_1$'s termination (line~\ref{line:rec_es_GC1_decide}), they immediately trigger their respective timer (line~\ref{line:rec_es_timeout1_measure}) that will expire within $2\delta$ time of each other. Let $\tau^{1}_e$ denote the time at which the first timer expires (line~\ref{line:rec_es_timer1_expires}). If $p_j$ proposes $(v, 1)$ to $\mathcal{EB}_{K_1}$, then $p_i$ proposes $(v, \cdot)$ to $\mathcal{EB}_{K_1}$, due to $\mathcal{GC}_{1}$'s consistency.

    \item $\mathcal{GC}_2$: Correct processes propose valid values to $\mathcal{GC}_2$ as a correct process proposes either (line~\ref{line:rec_es_GC2_propose_after_EB}) the output of $\mathcal{EB}_{K_1}$, which is externally valid due to $\mathcal{EB}_{K_1}$'s external validity or (line~\ref{line:rec_es_GC2_propose_after_timer}) $\mathcal{GC}_1$'s output which is valid due to $\mathcal{GC}_1$'s external validity. They do so within $2\delta$ time of each other. If a correct process proposes a value because of the timer expiration, it does so between $\tau^{1}_e$ and $\tau^{1}_e + 2\delta$. Assume a correct process proposes (line~\ref{line:rec_es_GC2_propose_after_EB}) a value coming from $\mathcal{EB}_{K_1}$. It necessarily does so before $\tau^{1}_e + 2\delta$. Let $\tau'' \leq \tau^{1}_e + 2\delta$ be the time at which the first correct proposes a value coming from $\mathcal{EB}_{K_1}$. By $\mathcal{EB}_{K_1}$'s totality, every correct process proposes (line~\ref{line:rec_es_GC2_propose_after_EB} or line~\ref{line:rec_es_GC2_propose_after_timer}) a value to $\mathcal{GC}_2$ between $\mathsf{min}(\tau^{1}_e, \tau'')$ and $\mathsf{min}(\tau^{1}_e, \tau'') + 2 \delta$.

    \item $\mathcal{F}_2$: Correct processes propose (line~\ref{line:rec_es_fin2_to_finish}) valid values to $\mathcal{F}_2$ because of $\mathcal{GC}_2$'s external validity. The simulation (each $\mathcal{GC}_2$'s round lasts $3\delta$) implies they do so within $2\delta$ time of each other. If $p_j$ proposes $(v, 1)$ to $\mathcal{F}_{2}$, then $p_i$ proposes $(v, \cdot)$ to $\mathcal{F}_{2}$, due to $\mathcal{GC}_{2}$'s consistency. Then, they wait for $3\delta$ time (line~\ref{line:rec_es_wait2}) before (i) triggering (line~\ref{line:rec_es_timeout2_measure}) their respective timer that will expire within $2\delta$ time of each other, and (ii) proposing (line~\ref{line:rec_es_EB2_input}) valid values to $\mathcal{EB}_{K_2}$ (the same as the one proposed to $\mathcal{F}_{2}$ line~\ref{line:rec_es_fin2_to_finish}) within $2\delta$ time of each other. Let $\tau^{2}_e$ denote the time at which the first timer expires (line~\ref{line:rec_es_timer2_expires}).

    \item $\mathcal{EB}_{K_2}$: As shown above, correct processes propose (line~\ref{line:rec_es_EB2_input}) valid values to $\mathcal{EB}_{K_2}$ within $2\delta$ time of each other. %Upon $\mathcal{GC}_2$'s termination, they immediately trigger their respective timer that will expire within $2\delta$ time of each other. 
    If $p_j$ proposes $(v, 1)$ to $\mathcal{EB}_{K_2}$, then $p_i$ proposes $(v, \cdot)$ to $\mathcal{EB}_{K_2}$, due to $\mathcal{GC}_{2}$'s consistency.

    \item Decision: Let $p$ be the first correct process that decides (line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, or line~\ref{line:recursive_early_stopping_decide_after_second_finisher}, or line~\ref{line:rec_es_decide_after_EB2} or line~\ref{line:rec_es_decide_after_timer2}), and does so by time $\tau^{d}$. ($\tau^{d} = \infty$ if no correct process ever decides). If $p$ decides line~\ref{line:recursive_early_stopping_decide_after_first_finisher} upon triggering $\mathcal{F}_1.\mathsf{advance}$ (line~\ref{line:rec_es_fin1_to_finish}) or line~\ref{line:recursive_early_stopping_decide_after_second_finisher} upon triggering $\mathcal{F}_2.\mathsf{advance}$ (line~\ref{line:rec_es_fin2_to_finish}), then every correct process decides by time $\tau^d + 2\delta$, due to finisher's totality. If $p$ decides line~\ref{line:rec_es_decide_after_EB2} upon outputting a value from $\mathcal{EB}_{K_2}$ line~\ref{line:rec_es_EB2_output}, then every correct process decides by time $\tau^d + 2\delta$, due to elector broadcast's totality. If $p$ decides line~\ref{line:rec_es_decide_after_timer2} upon $\mathit{timer}_2$'s expiration (line~\ref{line:rec_es_timer2_expires}), i.e. $\tau^d = \tau^{2}_e$, then every correct process decides by time $\tau^d + 2\delta$, since their respective timer expire within $2\delta$ time of each other.
    In each case, the decision is externally valid due to the external validity property of $\mathcal{F}_1, \mathcal{F}_2, \mathcal{GC}_2$, and $\mathcal{EB}_{K_2}$.
\end{compactitem}
\end{proof}

%% %% %%
%%%%%%%%





%The previous lemma shows that $\mathcal{GC}_0$, $\mathcal{GC}_1$ and $\mathcal{GC}_2$ work according to their specification (see \Cref{subsubsection:graded_consensus}) as correct processes only propose valid values.

We are ready to prove that \nameES satisfies strong validity.

\begin{theorem}[Strong validity]\label{lemma:rec_es_strong_validity}
\nameES satisfies strong validity.
\end{theorem}
\begin{proof}
Suppose that all correct processes propose the same value $v$ within $2\delta$ time of each other line~\ref{line:rec_es_propose}. Then, the post-conditions of \Cref{lemma:res_spec_assumption} are all verified.
Due to the strong validity property of $\mathcal{GC}_0$, all correct processes decide $(v, 1)$ from $\mathcal{GC}_{sv}$ line~\ref{line:rec_es_GCsv_decide}.
Due to the stability property of $\mathcal{EB}_{\{p_\ell\}}$, any correct process that outputs a value from $\mathcal{EB}_{\{p_\ell\}}$ line~\ref{line:rec_es_EBl_output}, does so with value $v$.
Thus, all correct processes propose $v$ to $\mathcal{GC}_\ell$, either line~\ref{line:rec_es_GCl_propose_after_EBL} as the output of $\mathcal{EB}_{\{p_\ell\}}$ or line~\ref{line:rec_es_GCl_propose_after_timer} as the output of $\mathcal{GC}_{sv}$ if the corresponding timer expires first line~\ref{line:rec_es_timer0_expires}.
Due to the strong validity property of $\mathcal{GC}_{\ell}$, all correct processes decide $(v, 1)$ from $\mathcal{GC}_\ell$ line~\ref{line:rec_es_GCl_decide}. Hence, all correct processes propose $(v,1)$ to $\mathcal{F}_1$ line~\ref{line:rec_es_fin1_finish}.
By $\mathcal{F}_1$'s liveness, all correct processes decide $v$ line~\ref{line:recursive_early_stopping_decide_after_first_finisher} from $\mathcal{F}_1$ and halt, before any process finishes the $3\delta$ waiting step (line~\ref{line:rec_es_wait_1}).
\end{proof}

%%%%%%%%
%% %% %%
\begin{lemma}\label{lemma:deciding_immediately_with_a_correct_leader}
    If process $p_\ell$ is correct, correct processes agree on a common value after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} by $O(\delta)$ time, without executing $\mathcal{GC}_1$.
\end{lemma}
\begin{proof}
    Assume $p_\ell$ is correct. Then, every correct process outputs the same value $v$ from $\mathcal{EB}_\ell$ line~\ref{line:rec_es_EBl_output} before $\mathit{timer}_0$'s expiration (line~\ref{line:rec_es_timer0_expires}). Hence, all correct processes propose $v$ to $\mathcal{GC}_1$ within $2\delta$ time of each other line~\ref{line:rec_es_GC1_propose}. Due to $\mathcal{GC}_1$'s consistency, every correct process outputs $(v,1)$ from $\mathcal{GC}_1$ line~\ref{line:rec_es_GC1_decide}. This means that all correct processes propose $(v,1)$ to $\mathcal{F}_1$ within $2\delta$ time of each other line~\ref{line:rec_es_fin1_to_finish}. Finally, due to $\mathcal{F}_1$'s liveness, every correct process outputs $v$ from $\mathcal{F}_1$ line~\ref{line:rec_es_fin1_finish},decides $v$ and halt at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} before the end of the $3\delta$-waiting step (line~\ref{line:rec_es_wait_1}).
\end{proof}

\begin{lemma}\label{lemma:deciding_via_finisher_implies_unanimity}
    If a correct process decides some value $v$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} (resp., second finisher $\mathcal{F}_2$ at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}), then every correct process that outputted from $\mathcal{GC}_\ell$ (resp., $\mathcal{GC}_2$), did so with pair $(v, \cdot)$.
\end{lemma}
\begin{proof}
    Assume a correct process decides $v$ line~\ref{line:recursive_early_stopping_decide_after_first_finisher} (resp., line~\ref{line:recursive_early_stopping_decide_after_second_finisher})  upon getting an output line~\ref{line:rec_es_fin1_finish} (resp., line~\ref{line:rec_es_fin2_finish}) from $\mathcal{F}_1$ (resp., $\mathcal{F}_2$). By finisher's justification, some correct process inputs $(v',1)$ to $\mathcal{F}_1$ (resp., $\mathcal{F}_2$) line~\ref{line:rec_es_fin1_to_finish} (resp., line~\ref{line:rec_es_fin2_to_finish}). By consistency property of $\mathcal{GC}_\ell$ (resp., $\mathcal{GC}_2$), every correct process that has outputted a pair to $\mathcal{GC}_\ell$ (resp., $\mathcal{GC}_2$) line~\ref{line:rec_es_GCl_decide} (resp., line~\ref{line:rec_es_GC2_decide}), did so with a pair $(v, \cdot)$.
\end{proof}

\begin{lemma}\label{lemma:first_finisher_preserves_agreement}
    If a correct process decides some value $v$ at time $\tau$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, then every correct process decides $v$ by time $\tau + 2\delta$.
\end{lemma}
\begin{proof}
    If a correct process decides some value $v$ at time $\tau$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, then every correct process that outputted from $\mathcal{GC}_\ell$, did so with pair $(v, \cdot)$. Thus, due to $\mathcal{GC}_1$'s strong validity, no correct process outputs a pair different from $(v,1)$ from $\mathcal{GC}_1$. Hence, no correct process can decide a value different from $v$, due to strong validity of $\mathcal{GC}_2$ and stability of $\mathcal{EB}_{K_2}$. Moreover, by $\mathcal{F}_1$'s totality, every correct process decides $v$ by time $\tau + 2\delta$.
\end{proof}

\begin{lemma}\label{lemma:early_stopping_with_an_healthy_first_half}
    If $K_1$ counts $f_1 < |K_1|/3$ faulty processes, correct processes agree on a common value by time $O(\delta) + \mathcal{L}_{\mathcal{BA}_{K_1}}(|K_1|, f_1)$, without executing $\mathcal{EB}_{K_2}$.
\end{lemma}
\begin{proof}
If a correct process decides some value $v$ at time $\tau$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, then every correct process decides $v$ by time $\tau + 2\delta$, due to \Cref{lemma:first_finisher_preserves_agreement}.
Assume no correct process decides after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} by time $\tau \in O(\delta) + \mathcal{L}_{\mathcal{BA}_{K_1}}(|K_1|, f_1)$.
Hence, all correct processes participate to $\mathcal{EB}_{K_1}$ within $2\delta$ of each other by time $\tau'$. Due to the agreement property and liveness property of $\mathcal{EB}_{K_1}$, all correct processes output (line~\ref{line:rec_es_EB1_output}) some value $v'$ from $\mathcal{EB}_{K_1}$ by time $\tau' + \mathcal{L}_{\mathcal{BA}_{K_1}}(|K_1|, f_1)$. Thus, all correct processes propose $v'$ to $\mathcal{GC}_2$ line~\ref{line:rec_es_GC2_propose_after_EB}, which means, due to $\mathcal{GC}_2$'s strong validity and $\mathcal{F}_2$'s liveness that all correct processes decide \ref{line:recursive_early_stopping_decide_after_second_finisher} a common value by time $O(\delta) + \mathcal{L}_{\mathcal{BA}_{K_1}}(|K_1|, f_1)$ before the end of the $3\delta$-waiting step (line~\ref{line:rec_es_wait2}).

In all cases, correct processes decide a common value by time $O(\delta) + \mathcal{L}_{\mathcal{BA}_{K_1}}(|K_1|, f_1)$ without executing $\mathcal{EB}_{K_2}$.

\end{proof}

\begin{lemma}\label{lemma:rec_es_agreement}
    \nameES satisfies agreement.
\end{lemma}
\begin{proof}
    If $p_\ell$ is correct or $K_1$ is healthy, we are done due to \Cref{lemma:deciding_immediately_with_a_correct_leader} and \Cref{lemma:early_stopping_with_an_healthy_first_half}. Assume $p_\ell$ is faulty and $K_1$ is not healthy. Hence, $K_2$ is healthy.
If a correct process decides some value $v$ at time $\tau$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}, then every correct process decides $v$ by time $\tau + 2\delta$, due to \Cref{lemma:first_finisher_preserves_agreement}.
Assume no correct process decides after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher}.

If some correct process decides after the second finisher $\mathcal{F}_2$ at line~\ref{line:recursive_early_stopping_decide_after_second_finisher} by time $\tau_2$, then due to \Cref{lemma:deciding_via_finisher_implies_unanimity}, every correct process outputs $(v,\cdot)$ from $\mathcal{GC}_{K_2}$ line~\ref{line:rec_es_GC2_decide}. Then, by $\mathcal{EB}_{K_2}$'s optimistic consensus, every correct process either outputs $v$ from $\mathcal{EB}_{K_2}$ line~\ref{line:rec_es_EB2_output} or first decides $v$ after the second finisher $\mathcal{F}_2$ at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}.

Assume no correct process decides after the second finisher $\mathcal{F}_2$ at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}. Then, by $\mathcal{EB}_{K_2}$'s optimistic consensus, all correct processes agree line~\ref{line:rec_es_decide_after_EB2} on some common value.
\end{proof}

%% %% %%
%%%%%%%%
We have shown that \nameES ensures all the properties of Byzantine agreement.

\begin{theorem}\label{theorem:nameES_solves_BA}
    \nameES solves Byzantine agreement.
\end{theorem}
\begin{proof}
    Agreement is ensured by \Cref{lemma:rec_es_agreement}, strong validity is guaranteed by \Cref{lemma:rec_es_strong_validity} and \Cref{lemma:res_spec_assumption} implies termination and external validity.
\end{proof}
    


Finally, we prove \nameES's complexity.

\begin{theorem} [Complexity] \label{theorem:nameES_complexity}
\nameES achieves $O\big( (L+n)\log(n) \big)$ per-process bit complexity and $O(\delta(f+1))$ latency.
%\nameES achieves $O\big( n \log(f+2) L + n^2 \log(n) \big)$ bit complexity and $O(\delta(f+1))$ latency.
\end{theorem}
\begin{proof}
The per-process bit complexity (resp., latency) of $\nameES$ among $n$ processes with $f$ actual failures, denoted as $\mathcal{B}(n,f)$ (resp., $\mathcal{L}(n,f)$), can be expressed differently for three cases:

1. $p_\ell$ is correct,
2. $p_\ell$ is faulty but $K_1$ is healthy, and
3. $p_\ell$ is faulty, $K_1$ is not healthy but $K_2$ is healthy.
We note $f_1$ (resp., $f_2$) the number of actual faulty processes in $K_1$ (resp., $K_2$).
Let us note that $f=1+f_1+f_2$ if $p_\ell$ is faulty. %\ayaz{$f_1, f_2 < f$. This fact is also important to understand why we don't need to spend $\Omega(\log n)$ rounds even if $f \in O(1)$, as shown in the latency proof (without step involving $p_\ell$, $f_1, f_2 \le f$)}

%The bit complexity for each case can be expressed as follows where $q_b$ and $\tilde{q}_b$ are constant:
% \begin{equation*}
% \mathcal{B}(n,f) =
% \begin{cases}
% O\big( nL + n^2 \log(n) \big) & \text{if $p_\ell$ is correct,} \\
% O\big( nL + n^2 \log(n) \big) + \mathcal{B}(\frac{n}{2},f_1) & \text{if $p_\ell$ is faulty but $K_1$ is healthy,} \\
% O\big( nL + n^2 \log(n) \big) + \mathcal{B}(\frac{n}{2},f_1) + \mathcal{B}(\frac{n}{2},f_2) & \text{otherwise.}
% \end{cases}
% \end{equation*}

The per-process bit complexity verifies the following inequality where $a$ and $b$ are some positive constants related to the different modules (with $aL + b\log (n) \geq 4\mathcal{B}_{\mathcal{GC}}(n) + 3\mathcal{B}_{\mathcal{CD}}(n) + 2\mathcal{B}_{\mathcal{F}}(n)$, where $\mathcal{B}_{\mathcal{M}}(n)$ denotes the worst-case per-process bit complexity of module $\mathcal{M}$ among $n$ processes, that can be graded consensus ($\mathcal{GC}$), committee-dissemination ($\mathcal{CD}$), and finisher ($\mathcal{F}$)):
% \begin{equation*}
% \mathcal{B}(n,f) \leq q_b L + \tilde{q}_b  \log(n) + \mathsf{max} \big( \mathcal{B}(\frac{n}{2}, f_1), \mathcal{B}(\frac{n}{2}, f_2) \big)
% \end{equation*}

\begin{equation*}
\mathcal{B}(n,f) \leq
\begin{cases}
0 & \text{if $n=1$} \\
a L + b  \log(n) & \text{if $p_\ell$ is correct,} \\
a L + b  \log(n) + \mathsf{max} \big( \mathcal{B}(\frac{n}{2}, f_1), \mathcal{B}(\frac{n}{2}, f_2) \big) & \text{otherwise}
\end{cases}
\end{equation*}




By induction, we will show that for every integer $n$, $\mathcal{B}(n,f) \leq c (L+n) \log (n)$ for some sufficiently large positive constant $c\geq \mathsf{max}(2b, a/\log(2))$. The base case trivially holds since $\mathcal{B}(1,0) = 0$. Let $n$ be a strictly positive integer. We assume the result holds for any integer stritcly lower than $n$.
By the induction hypothesis,
$\mathsf{max}\big(\mathcal{B}(\frac{n}{2}, f_1), \mathcal{B}(\frac{n}{2}, f_2)\big) \leq c(L+\frac{n}{2})\log (\frac{n}{2} )$.
Hence, $\mathcal{B}(n,f) \leq (a-c\log(2)+c\log(n))L + (b+\frac{c}{2})n\log(n)$.
Finally, $\mathcal{B}(n,f) \leq c (L+n) \log (n)$, since $c\geq \mathsf{max}(2b, a/\log(2))$. The induction holds, which concludes the proof for the per-process bit complexity.

% %$\mathcal{B}(n,f) \leq q_b nL + \tilde{q}_b n^2 \log(n) + \mathcal{B}(\frac{n}{2}, f_1) + \mathcal{B}(\frac{n}{2}, f_2)$.
% First, we develop the induction hypothesis:
% $\forall i \in \{1,2\}, \mathcal{B}(\frac{n}{2}, f_i) \leq q_b' L \log (f_i)  + \tilde{q}'_b \frac{n}{2}   \log (\frac{n}{2} ) $.

% Hence, $\mathcal{B}(n, f) \leq (q_b + q'_b\log (f-1))L + (\tilde{q}_b + \tilde{q}'_b \frac{n}{2} )  \log (n) $ 

% \ayaz{The base case of the induction is $\mathcal{B}(1, f)$, where the hypothesis holds as when $n=1$ the complexity is $0$.}

% Since $f_1 f_2 \leq (f/2)^2$, $\mathcal{B}(\frac{n}{2}, f_1) + \mathcal{B}(\frac{n}{2}, f_2) \leq q_b' L (\log (f)-\log (2)) + \tilde{q}'_b n (\log (n) - \log (2) ) $. 

% Hence, $\mathcal{B}(n,f) \leq  L (q_b'\log (f)+q_b-\log (2)q_b')+ (\frac{\tilde{q}'_b}{2} + \tilde{q}_b) \log (n)$. 

% Since we have chosen $\tilde{q}'_b$ and $q'_b$ sufficiently large to verify
% (1) $\tilde{q}'_b > 2\tilde{q}_b$ and (2) $q_b' > q_b/ \log (2)$, we obtain $\mathcal{B}(n,f) \leq  nL (q_b'\log (f)) + \tilde{q}'_b n^2 \log (n)$, which terminates the induction and yields the result.  

% \ayaz{at some point, should we mention that this protocol has balanced communication complexity? (right now it is sort of mentioned in the intro)}

%Thus the result is immediate. \pierre{Can we achieve $O\big( n \log(f+2) L + n^2 \log(n) \big)$ bit complexity, i.e. optimality when $f=O(1)$ and $L = \Omega(n \log (n))$ ?}

Analogously, Let $\mathcal{L}_{\mathcal{M}}$ denotes the worst-case (independent of $n$) latency of module $\mathcal{M}$, that can be graded consensus ($\mathcal{GC}$), committee-dissemination ($\mathcal{CD}$), and finisher ($\mathcal{F}$)). Let $a'$, $b'$ and $c'$ be some constants verifying:
\begin{equation*}
\begin{cases}
a' = (1/\delta) * \big(2*3*\mathcal{L}_{\mathcal{GC}} + \mathcal{L}_{\mathcal{CD}} + \mathcal{L}_{\mathcal{F}} + 2\big) = (2*3*7 + 5 + 1 + 2) = 50 \\
b' = (1/\delta) * \big( 2*3*\mathcal{L}_{\mathcal{GC}} + \mathcal{L}_{\mathcal{CD}} + \mathsf{max}(\mathcal{L}_{\mathcal{CD}}, \mathcal{L}_{\mathcal{F}}) \big) = (2*3*7 + 5 + 5)  =  52  \\
c' = 2a' + b' = 152
\end{cases}
\end{equation*}


The latency of the recursive early stopping protocol can be expressed as follows:
\begin{equation*}
\mathcal{L}(n,f) \leq
\begin{cases}
a' \delta & \text{if $p_\ell$ is correct,} 
%\\ (a'+b') \delta + \mathcal{L}(\frac{n}{2},f_1) & \text{if $p_\ell$ is faulty but $K_1$ is healthy,} 
\\ (a'+b') \delta + \mathcal{L}(\frac{n}{2},f_1) + \mathcal{L}(\frac{n}{2},f_2) & \text{otherwise.}
\end{cases}
\end{equation*}
 


%\ayaz{If $f > n/3$, is $\mathcal{L}(n, f) = \mathcal{L}(n, n/3)$? through the use of the timer.}\pierre{yes}

By induction, we will show that $\mathcal{L}(n,f) \leq (a'+c'f)\delta$, where $c'$ is a sufficiently large positive constant: $c' \geq 2a' + b'$. 
Since  $\mathcal{L}(n,0) \leq a'\delta$ for any $n$,  the base case trivially holds. 
Let $n, f$ be two strictly positive integers.
We assume $\mathcal{L}(n',f') \leq (a'+c'f')\delta$ for any pair $(n',f')$ such that either $n' < n$ and $f' \leq f$ or $n' \leq n$ and $f' < f$, and aim to show it implies the result for the pair $(n,f)$. 



%\ayaz{Does $\tilde{q}$ also takes into account the committee disseminations inside of the elector broadcasts?}\pierre{yes}

%\ayaz{Base case is $\mathcal{L}(1, f)$ and $\mathcal{L}(n, 0)$, where $a'\delta$ latency occurs (matching the hypothesis).}

\begin{itemize}
    \item Case 1: $p_\ell$ is correct. The result immediately holds.

      \item Case 2: $p_\ell$ is faulty. In this case, $f=1+f_1+f_2$. Hence, by induction hypothesis, both $\mathcal{L}(\frac{n}{2},f_1) \leq (a'+c'f_1)$ and $\mathcal{L}(\frac{n}{2},f_2) \leq (a'+c'f_2)$ and thus, $\mathcal{L}(\frac{n}{2},f_1) + \mathcal{L}(\frac{n}{2},f_2) \leq (2a'-c'+c'f)$.
      
      This implies $\mathcal{L}(n,f) \leq (a'+b') \delta + \mathcal{L}(\frac{n}{2},f_1) + \mathcal{L}(\frac{n}{2},f_2) \leq a' \delta + (b'+2a'-c'+c'f)\delta \leq a' \delta + c'f\delta$.
\end{itemize}




 


%assume $\mathcal{L}(\frac{n}{2}, f_1) \leq (q_a + q_b f_1)\delta$ with $q_a \leq q$. Thus, if $p_\ell$ is correct $\mathcal{L}(n, f) = \mathcal{L}(\frac{n}{2}, f_1) = (q_a + q_b f_1)\delta$
%$\mathcal{L}(n, f) = \mathcal{L}(\frac{n}{2}, f_1) = (q_a + q_b f_1)\delta$

The induction is proven in all cases. Therefore, the proof is concluded.
\end{proof}



% \begin{lemma}
%     If a correct process decide some value $v$ after the first finisher $\mathcal{F}_1$ at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} (resp., second finisher $\mathcal{F}_2$ at line~\ref{line:recursive_early_stopping_decide_after_second_finisher}), then every correct process decide $v$.
% \end{lemma}
% \begin{proof}
% Assume a correct process decide some value $v$ after the first (resp., second) finisher $\mathcal{F}_1$ (resp., $\mathcal{F}_2$) at line~\ref{line:recursive_early_stopping_decide_after_first_finisher} (resp., line~\ref{line:recursive_early_stopping_decide_after_second_finisher}). Due to lemma \cite{lemma:deciding_via_finisher_implies_unanimity}, every correct process that that outputs from $\mathcal{GC}_1$ (resp., $\mathcal{GC}_2$), does so with pair $(v, \cdot)$.
% \end{proof}

% %%%

% The following lemma proves that if $p_1$ is correct, then correct processes decide a common externally valid value without executing $\mathcal{EB}_{K_1}$, $\mathcal{GC}_{2}$, $\mathcal{F}_{2}$, and $\mathcal{EB}_{K_2}$.

% \begin{lemma}
%     If $p_1$ is correct, then correct processes decide the same externally valid value. Moreover, they do not  execute $\mathcal{EB}_{K_1}$, $\mathcal{GC}_{2}$, $\mathcal{F}_{2}$, and $\mathcal{EB}_{K_2}$.
% \end{lemma}
% \begin{proof}
%     By agreement property of $\mathcal{EB}_{\{p_1\}}$, correct processes output the same value $v$ from $\mathcal{EB}_{\{p_1\}}$, and input $v$ to $\mathcal{GC}_{1}$. By $\mathcal{GC}_{1}$'s strong validity, all correct processes output $(v,1)$ from $\mathcal{GC}_{1}$ and input $(v,1)$ to $\mathcal{F}_{1}$ in some time window $[\tau, \tau+2\delta]$. By $\mathcal{F}_{1}$'s liveness, all correct processes decide $v$ from $\mathcal{F}_{1}$ in some time window $[\tau+\delta, \tau+3\delta]$. They immediately decide $v$ and halt. Thanks to the $3\delta$-waiting step, no correct process executes $\mathcal{EB}_{K_1}$, $\mathcal{GC}_{2}$, $\mathcal{F}_{2}$, or $\mathcal{EB}_{K_2}$.
% \end{proof}

% Similarly, we prove that if $K_1$ is healthy, then correct processes decide a common externally valid value without executing $\mathcal{EB}_{K_2}$.

% \begin{lemma}
%     If $K_1$ is healthy, then correct processes decide the same externally valid value with $2\delta$ time of each other. Moreover, they do not  execute $\mathcal{EB}_{K_2}$.
% \end{lemma}
% \begin{proof}
%     Correct processes output from $\mathcal{GC}_1$ with $2\delta$ time of each other. Since $K_1$ is healthy, correct processes cannot see their corresponding timers expire before obtaining a value from $\mathcal{EB}_{K_1}$. Hence, every correct process either input to $\mathcal{GC}_2$ the value obtained from $\mathcal{EB}_{K_1}$, or has decided and halted before after having outputted from $\mathcal{F}_1$.

%    Assume no correct process outputs from $\mathcal{F}_1$. By agreement property of $\mathcal{EB}_{K_1}$, correct processes output the same value $v$ from $\mathcal{EB}_{K_1}$, and input $v$ to $\mathcal{GC}_{2}$. By $\mathcal{GC}_{2}$'s strong validity, all correct processes output $(v,1)$ from $\mathcal{GC}_{2}$ and input $(v,1)$ to $\mathcal{F}_{2}$ in some time window $[\tau, \tau+2\delta]$. By $\mathcal{F}_{2}$'s liveness, all correct processes decide $v$ from $\mathcal{F}_{2}$ in some time window $[\tau+\delta, \tau+3\delta]$. They immediately decide $v$ and halt. Thanks to the $3\delta$-waiting step, no correct process executes $\mathcal{EB}_{K_2}$.

%    Assume a correct process decide $v$ upon getting an output from $\mathcal{F}_1$. 
%     By $\mathcal{F}_1$'s justification, some correct process inputs $(v',1)$ to $\mathcal{F}_1$.
%     By $\mathcal{GC}_1$'s consistency, every correct process inputs $(v,\cdot)$ to $\mathcal{F}_1$. By $\mathcal{F}_1$'s integrity, every correct process that outputs from $\mathcal{F}_1$, does so with value $v$. 
%     In parallel, correct processes that input to $\mathcal{EB}_{K_1}$, do so with value $v$. Hence, by strong validity and agreement of $\mathcal{EB}_{K_2}$, correct  processes that output from $\mathcal{EB}_{K_1}$, do so with value $v$. By $\mathcal{GC}_2$'s strong validity, every correct process that inputs to $\mathcal{F}_2$, does so with value $(v,1)$. Hence, correct processes decide $v$ and halt within $2\delta$ time of each other (either upon getting an output from $\mathcal{F}_1$ or from $\mathcal{F}_2$, due to the totality property of $\mathcal{F}_1$ and $\mathcal{F}_2$). The external validity of $v$ is guaranteed by external validity of $\mathcal{F}_1$ and $\mathcal{F}_2$ and lemma \ref{lemma:res_spec_assumption}.
    
%     %By $\mathcal{F}_1$'s totality, correct processes correct decide in a time window $[\delta, 2\delta]$.
% \end{proof}

% Analogously, we prove that if $K_2$ is healthy, then correct processes decide a common externally valid value within $2\delta$ time of each other.

% \begin{lemma}
%     If $K_2$ is healthy, then correct processes decide the same externally valid value within $2\delta$ time of each other. 
% \end{lemma}

==> sections/related_work.tex <==
\section{Related Work}\label{section:related_work}

% We address the communication complexity of deterministic signature-free Byzantine consensus~\cite{Lamport1982,Cachin2001} in synchronous  distributed systems for large inputs.
% Here, we discuss existing results in closely related contexts, and provide a brief overview of techniques, tools and building blocks which are often employed to tackle Byzantine consensus.\footnote{We use ``consensus'' and ``agreement'' interchangeably.}

% \smallskip
\noindent \textbf{Graded consensus.}
% Following the seminal Dolev-Reischuk lower bound~\cite{dolev1985bounds} stating that $\Omega(nt)$ messages must be exchanged for solving Byzantine agreement, Abraham and Stern~\cite{AbrahamStern22} have proven that graded consensus also requires $\Omega(nt)$ exchanged messages (assuming that $L \in O(1)$).
Graded consensus and other closely related problems such as (binding) (graded) crusader agreement~\cite{ABY22,MostefaouiMR15} have been collectively studied by Attiya and Welch~\cite{AW23}, who refer to this family of problems as ``connected consensus''.
In brief, connected consensus can be viewed as approximate agreement on spider graphs, consisting of a central clique (could be a single vertex) to which different paths (“branches”) are attached, each representing a potential value.

Graded consensus and the related problems have proven extremely helpful for solving Byzantine agreement.
In fully asynchronous environments, an alternating sequence of quadratic instances of binding crusader agreement and (reasonably fair) common coin allows for a binary Byzantine agreement with strong validity, an expected $O(n^2)$ bit complexity and an expected $O(1)$ latency~\cite{ABY22,MostefaouiMR15}.
In synchrony, graded consensus has been employed in various adaptions of the ``phase king'' methodology~\cite{Lenzen2022,CoanW92,berman1992bit,Momose2021} to achieve quadratic consensus for constant-sized values.

Following the seminal Dolev-Reischuk lower bound~\cite{dolev1985bounds} stating that $\Omega(nt)$ messages must be exchanged for solving Byzantine agreement, Abraham and Stern~\cite{AbrahamStern22} have proven that binary crusader broadcast (and so graded consensus) also requires $\Omega(nt)$ exchanged messages (assuming that $L \in O(1)$).
When $L \in O(1)$, Attiya and Welch~\cite{AW23} present an optimally resilient ($t < n / 3$), error-free connected consensus algorithm with optimal $O(n^2)$ bit complexity even in asynchrony.
Momose and Ren~\cite{Momose2021} present a synchronous graded consensus algorithm secure against a computationally bounded adversary with (1) optimal resilience ($t < n / 2$), and (2) $O(n^2\kappa)$ bit complexity (again, for $L \in O(1)$), where $\kappa$ denotes the size of cryptographic objects.
However, for longer $L$-bit values, related work is not as rich.
Abraham and Asharov~\cite{Abraham2022} solve gradecast \cite{FeldmanMicali88},  with optimal $O(nL)$ bit complexity in synchrony, albeit with a statistical error (their protocol is not error-free). 
(Gradecast can be described as a sender-oriented counterpart of graded consensus, i.e., gradecast and graded consensus enjoy a similar relation as Byzantine agreement and Byzantine broadcast~\cite{PSL80,lamport2019concurrency}.)
%It is worth mentioning that gradecast can be derived from graded consensus with no asymptotical overhead in terms of exchanged bits.

As mentioned in \Cref{section:introduction}, our graded consensus implementation relies on the techniques introduced by Chen in the COOL protocol~\cite{Chen2021}.
Recall that COOL is an error-free synchronous Byzantine agreement algorithm that satisfies (only) strong validity, exchanges $O\big( nL + n^2 \log(n) \big)$ bits and terminates in $O(n)$ rounds.
The structure of COOL consists of four phases.
The first three phases reduce the number of possible decision values to at most one, i.e., only one value ``survives'' the first three phases.
At the end of the third phase, all processes engage in a one-bit Byzantine agreement algorithm to decide whether a non-$\bot$ or the $\bot$ value should be decided from COOL.
If it is decided that a non-$\bot$ value should be decided, all processes participate in the fourth, reconstruction phase whose goal is to allow all processes to obtain that one (non-$\bot$) value that has previously survived the first three phases.
% We emphasize that COOL can trivially be modified to obtain early stopping (terminating in $O(f)$ rounds, where $f \leq t$ is the actual number of failures) by employing the early-stopping one-bit agreement protocol presented in~\cite{Lenzen2022}.

% Li and Chen's development of COOL and A-COOL protocols \cite{Li2021,Chen2021} presents a notable advancement. 
% This protocol, which does not adhere to the ``phase king'' framework, offer quadratic, error-free extension protocols for BA and BB. They achieve optimal $n/3$ resiliency (resp. sub-optimal $n/5$ resiliency) within a synchronous (resp. asynchronous) network. Their focus is on strong validity, allowing for a non-value $\bot$ when not all correct processes propose an identical value. They implement a four-phase approach where the final phase, triggered for non-$\bot$ values, is a simple reconstruction phase with constant latency and no synchronization requirement. In addition, the first three phases also maintain constant latency, culminating in the execution of a 1-bit Byzantine agreement instance. Using the early-stopping protocol of \cite{Lenzen2022} in \cite{Chen2021} maintains the same communication complexity while enabling early stopping.

\add{\medskip 
\noindent \textbf{\textsc{Signature-based explicit proof of retrievability}.}
Using cryptographic-signatures, it is possible to build an explicit proof of retrievability (PoR), a.k.a proof of dispersal. This cryptographic object is typically a signature-based certificate that testifies correct processes collectively posses sufficient material to retrieve the pre-image of a particular digest. The objective then becomes to efficiently: (1) disperse long values, (2) ensure that each correct process acquires a PoR, (3) agree on a PoR, whose size is independant of $L$, via a seed validated Byzantine Agreement, (4) retrieve the pre-image of the corresponding digest. All these steps must be performed with $O(nL+\mathit{poly}(\kappa,n))$ communication complexity. This approach has been successfully realized in a plethora of different models with different subtle trade-offs \cite{Abraham2023a,ada_dare_to_appear_podc24,civit_et_al:LIPIcs.DISC.2023.13,Lu2020,Nayak2020}. Importantly, this approach requires signatures to render the PoR ``self-certifying''. This means that determining the retrievability of a digest's pre-image does not rely on other information gathered in a specific sub-protocol.  Without such ``external verifiability'', correct processes may have differing guesses about the retrievability of a digest. If there is no consensus among these opinions, we cannot reduce the problem to a single MVBA designed for small values.
 
The natural approach to adapt this method is:

(1) each process $p_i$ computes $n$ Reed-Solomon shares $[s_i^1, ..., s_i^n]$ of its proposal value $v_i$ and the merkle root $D_i$ of the merkle tree whose leaves consist of $\{(1,s_i^1), ..., (n,s_i^n)\}$ and the corresponding merkle proofs (witnesses) $\{w_i^1, ..., w_i^n\}$. Then it sends $(D_i, s_i^j, w_i^j)$ to each process and use a succinct interactive argument (SIARG (or computationally sound proof system)) protocol to convince each correct process that $D_i$'s pre-image $v_i$ is externally valid. 

(2) Processes participate in $n$ parallel instances of byzantine broadcast (using $\kappa$-parallel byzantine broadcast implemented by \cite{Lenzen2022}), where the leader of instance $BB_j$ is process $p_j$ and inputs $D_j$.

(3) Each correct process broadcasts its opinion about the correctness of each other process. 

(4) Processes participate in $n$ parallel instances of a binary agreement (using \cite{Lenzen2022}). For each instance $BBA_j$, a process proposes $1$ if it received $n-t$ positive opinions about process $p_j$ in the second phase, and $0$ otherwise. 

(5) A correct process considers that digest $D_j$ received in $BB_j$ is retrievable iff it outputs $1$ from $BBA_j$. 

(6) Correct processes participate to a MVBA designed for $\kappa$-bits values (we can trivially adapt the protocol of \cite{Lenzen2022} to achieve $O(\kappa n^2)$ complexity and $O(f+1)$ latency), where the validity predicate corresponds to the retrievability established in (4).

(7) Upon deciding a digest $D^*$, correct processes reconstruct the corresponding pre-image atop the shares collect in (1). Indeed, if $D^*$ has been decided, it means it is valid according to the MVBA's validity predicate, so retrievable according to (5), which means $D^* = D_j$ with $BBA_j$ that returned $1$. By $BBA_j$'s strong validity, at least one correct process $p_k$ proposed $1$ to $BBA_j$ in (4), which means $p_k$ received $n-t$ positive opinions for process $p_j$, which means at least $t+1$ correct processes obtained the polynomial shares that are enough for the reconstruction of the pre-image (the witnesses prevent from receiving ill-fromed shares from Byzantine processes).
The latency is dominated by the $\Theta(f+1)$ latency of the BB/BA/MVBA agreement protocols. 
The communication complexity is dominated by (i) the $\Theta(\kappa n^3)$ bits exchange in step (3), and (ii) $n^2 B(SIARG)$, where $B(SIARG)$ is the bit complexity of the SIARG protocol.
%That is why \nameopt (and \name) is not an extension protocol relying on seed agreement protocol for smaller values. 
}

% \medskip 
% \noindent \textbf{\textsc{ADA-DARE}.}
% \textsc{ADA-DARE}~\cite{podc_2024_submission} solves the Byzantine agreement problem (with strong and external validity) while achieving near-optimal $O(nL + n^2\kappa)$ bit complexity, where $\kappa$ denotes the size of cryptographic objects, against a computationally bounded adversary.
% Importantly, \textsc{ADA-DARE} is optimally resilient $(t < n / 2)$, and is safe only against a computationally bounded adversary.
% \textsc{ADA-DARE} leverages concepts introduced in~\cite{cohen2023make,Momose2021,Nayak2020,rambaud2022linear}.

\medskip
\noindent \textbf{Randomized Byzantine agreement in synchrony against a computationally unbounded adversary.}
Without trusted-setup, Byzantine agreement is solvable against a computationally unbounded adversary if and only if $t < n / 3$~\cite{FLM85,PSL80,pfitzmann1996information}. 
Importantly, one can use $n$ parallel instances of the Byzantine broadcast primitive~\cite{PSL80} to solve Byzantine agreement.
(Byzantine broadcast is an agreement problem in which processes need to agree on the value held by one predetermined process.)
There exist randomized statistically secure (resilient against a computationally unbounded adversary with probability $1-\frac{1}{2^{\lambda}}$, where $\lambda$ represents some security parameter) Byzantine broadcast protocols that achieve sub-quadratic expected bit complexity (assuming $L \in O(1)$).
However, these algorithms either (1) tackle only static adversaries that corrupt processes at the beginning of an execution~\cite{King2006a,King2009,braud2013fast,Gelles23},\footnote{We underline that \name, as it is a deterministic protocol, tolerates an adaptive adversary capable of corrupting processes during (and not only before) any execution (see \Cref{section:preliminaries}). 
This remains true even if such an adaptive adversary is equipped with after-the-fact-removal capabilities~\cite{AbrahamRevisited,Abraham2023revisited}.} or (2) require private (also known as secure) communication channels~\cite{King2009}.
Facing static corruption only, there exists a solution to the Byzantine agreement problem that does not rely on $n$ instances of Byzantine broadcast.
(1) Processes agree (with high probability) on a $\lambda$-sized committee, which then executes any Byzantine agreement protocol and disseminates the decided value to all processes outside the committee.
(2) A non-committee process decides on the majority value.
This protocol is correct as long as there is a correct majority in the committee, that is with probability $1-\mathit{exp}(-\Omega(\lambda))$ due to the standard Chernoff bound.
% \ayaz{is there a paper we can cite about this?}\jovan{Not that I am aware. This was just a toy solution that can be obtained.}\ayaz{yep agree on that}

% \paragraph*{Randomized and/or signature-based Byzantine brodcast protocols}

% Achieving $t$-resiliency where $t>n/3$ implies that the system can only tolerate a bounded adversary \cite{FLM85}.
% Sub-quadratic randomized Byzantine Broadcast protocols can tolerate a computationally bounded, though adaptive, adversary \cite{chen2019algorand,AbrahamRevisited}.
% Interestingly, it's feasible to deterministically manage 
% up to $t=n-1$ adaptive Byzantine corruptions through the use of simple digital signatures \cite{Dolev1983}. Moreover, recent advancements have achieved sub-cubic expected communication complexity in the dishonest majority regime (i.e., $t>n/2$)  \cite{Chan2020,Tsimos2022}.

% In scenarios where $t<n/3$, addressing an unbounded adversary becomes possible. There are randomized information theoretic protocols that achieve sub-quadratic expected complexity. However, these protocols are typically designed to counter static adversaries \cite{King2006a,King2009,braud2013fast,Gelles23} or rely on private (also known as secure) communication channels \cite{King2009}.

% Regarding deterministic protocols, their design inherently means they do not differentiate when confronting a strongly adaptive equipped with after-the-fact-removal capabilities \cite{AbrahamRevisited,Abraham2023revisited}. 

% In the honest-majority regime, we know of several protocols, deterministic
% \cite{berman1992bit,CoanW92,Momose2021}, or randomized \cite{micali2017very,fitzi2021new}, that match the known lower bounds \cite{Dolev1985,AbrahamRevisited,Abraham2023revisited} for strongly adaptive adversaries. 
% When considering static, or weakly adaptive security, a fruitful line of works achieved sub-quadratic communication, with information-theoretic security 
% \cite{King2006a,King2009,King2011,braud2013fast} 
% or with computational security \cite{chen2019algorand,AbrahamRevisited,Cohen2020,cohen2020not,Blum2020,Boyle2021}. 

% \cite{King2006a}: static adversary
% \cite{King2009}: static adversary
% \cite{King2011}: private channels
% \cite{braud2013fast}: static adversary
% \cite{Gelles23} : static adversary

% In the dishonest-majority regime, the most communication-efficient broadcast constructions are
% based on the protocol of Dolev and Strong \cite{Dolev1983}. This protocol is secure facing any number of strongly adaptive corruptions and the communication complexity is $O(n^3)$. When considering weakly adaptive corruptions, Chan et al. \cite{Chan2020} used cryptography and trusted setup to dynamically elect a small, polylog-size committee in each round and improved the communication to $\tilde{O}(n^2)$. In the static-corruption setting, Tsimos et al. \cite{Tsimos2022} achieved $\tilde{O}(n^2)$ communication by
% running the protocol of \cite{Dolev1983} over a “gossiping network” 
% \cite{demers1987epidemic,karp2000randomized}. This work further achieved amortized sub-quadratic communication facing weakly adaptive corruptions when all parties broadcast in parallel.

% \smallskip
% \noindent \textbf{Extension protocols}
% \cite{Nayak2020,Ganesh2016,Ganesh2017,Ganesh2021}.
% An extension protocol optimizes for long inputs via a reduction to the same problem with small inputs (considered an oracle).
% Using extension protocols, several state-of-the-art results were achieved in the authenticated and unauthenticated models, both in synchronous and fully asynchronous settings for Byzantine consensus, Byzantine broadcast and reliable broadcast \cite{Nayak2020}. 
% Applying the extension protocol of \cite{Nayak2020} to \cite{Momose2021}, synchronous Byzantine agreement can be implemented with optimal resiliency ($t<n/2$) and a bit complexity of $O(nL + n^2\kappa)$.
% Interestingly, it has been demonstrated that synchronous Byzantine agreement can be implemented with a bit complexity of $O(n (L+\mathit{poly}(\kappa)))$ using randomization \cite{Bhangale2022}. The Dolev-Reischuk bound \cite{Dolev1985} is not violated in this case since the implementation tolerates a negligible (with $\kappa$) probability of failure, whereas the bound holds for deterministic protocols.
% In asynchrony, by applying the (asynchronous) extension protocol of \cite{Nayak2020} to \cite{abraham2019asymptotically}, the same asymptotic result as \cite{Lu2020} is achieved, solving asynchronous MVBA with an expected bit complexity of $O(nL + n^2\kappa)$.

% Unconditionally secure Byzantine agreement with large inputs has been addressed by \cite{Chen2020, Chen2021} under synchrony and \cite{Li2021} under asynchrony, assuming a common coin (implementable via unconditionally-secure Asynchronous Verifiable Secret Sharing~\cite{Choudhury2023}).
% Despite \cite{kaklamanis2022} utilizing erasure codes to alleviate leader bottleneck, and the theoretical construction of \cite{validity_paper} with exponential latency, there is, to the best of our knowledge, no viable extension protocol for Byzantine agreement in partial synchrony achieving results similar to ours ($o(n^2L)$).

\smallskip
\noindent \textbf{Error correction.}
Many distributed tasks~\cite{das2021asynchronous,Yurek2022,Shoup2023,Choudhury2023,Das2022,Gagol2019,Keidar2021,Camenisch2022,Duan2022,Abraham2022,Lu2020,Nayak2020} employ coding techniques such as erasure codes~\cite{blahut1983theory, Hendricks2007b, alhaddad2021succinct} or error-correction codes~\cite{reed1960, BenOr1993}.
For the comprehensive list of distributed primitive utilizing coding techniques, we refer the reader to \cite{civit_et_al:LIPIcs.DISC.2023.13}.


% (e.g., erasure codes~\cite{blahut1983theory, Hendricks2007b, alhaddad2021succinct} or error-correction codes~\cite{reed1960polynomial, BenOr1993}): Asynchronous Data Dissemination (ADD) \cite{das2021asynchronous}, Asynchronous Verifiable Secret Sharing (AVSS) against a computationally bounded \cite{das2021asynchronous, Yurek2022, Shoup2023} or unbounded \cite{Choudhury2023} adversary,
% Random Beacon \cite{Das2022}, Atomic Broadcast in both the asynchronous \cite{Gagol2019, Keidar2021} and partially synchronous \cite{Camenisch2022} settings, Information-Theoretic (IT) Asynchronous State Machine Replication (SMR) \cite{Duan2022}, Gradecast in synchrony and Reliable Broadcast in asynchrony \cite{Abraham2022}, Asynchronous Distributed Key Generation (ADKG) \cite{das2021asynchronous, Das2022b}, Asynchronous Verifiable Information Dispersal (AVID) \cite{Alhaddad2022}, Byzantine Storage \cite{Dobre2019, Androulaki2014, Hendricks2007}, Asynchronous Common Subset (ACS) \cite{duan2023practical}, and Multi-valued Validated Byzantine Agreement (MVBA) \cite{Lu2020, Nayak2020}.
% Coding techniques are often used to reduce the worst-case complexity by allowing a group of processes to balance and share the cost of sending a value to an individual (potentially faulty) node and are also used in combination with other techniques, such as commitment schemes \cite{catalano2013vector, Lu2020}.

% \smallskip
% \noindent {We now list several problems related to or used in solving Byzantine agreement.}

% \smallskip
% \noindent \textbf{Asynchronous Common Subset (ACS)}.
% The goal in ACS \cite{BenOr1993, ben1994asynchronous, duan2023practical} (also known as Vector Consensus \cite{neves2005solving,Doudou1998,correia2006consensus}) is to agree on a subset of $n - t$ proposals. 
% When considering a generalization of the validity property, this problem represents the strongest variant of consensus \cite{validity_paper}.
% Atomic Broadcast can be trivially reduced to ACS \cite{Doudou1998, Cachin2001, miller2016}. 
% There are well-known simple asynchronous constructions that allow for the reduction of ACS to either (1) Reliable Broadcast and Binary Byzantine Agreement \cite{ben1994asynchronous}, or (2) MVBA \cite{Cachin2001} in the authenticated setting, where the validation predicate requires the output to be a vector of signed inputs from at least $n-t$ parties.
% The first reduction enables the implementation of ACS with a cubic bit complexity, using the broadcast of \cite{Abraham2022}. 
% The second reduction could be improved further with a more efficient underlying MVBA protocol, such as \darestark.

% \smallskip
% \noindent \textbf{Asynchronous Verifiable Information Dispersal (AVID)}. 
% AVID \cite{cachin2005} is a form of "retrievable" broadcast that allows the dissemination of a value while providing a cryptographic proof that it can be retrieved. 
% This primitive can be implemented with a total dispersal cost of $O(L + n^2\kappa)$ bits exchanged and a retrieval cost of $O(L + n\kappa)$ per node, relying only on the existence of collision-resistant hash functions \cite{Alhaddad2022}. 
% AVID is similar to our Dispersal and Retrieval phases, but has two key differences.
% First, AVID's retrieval protocol only guarantees that a valid value will be retrieved if the original process dispersing the information was correct.
% Second, it is a broadcast protocol, having stricter delivery guarantees for each process.
% Concretely, if a correct process initiates the AVID protocol, it should eventually disperse its \emph{own} value.
% In contrast, we only require that a correct process obtains a proof of dispersal for \emph{some} value.

% \smallskip
% \noindent \textbf{Provable Broadcast (PB) and Asynchronous Provable Dispersal Broadcast (APDB)}.
% PB \cite{Abraham2019a} is a primitive used to acquire a succinct proof of external validity. 
% It is similar to our Dispersal phase, including the algorithm itself, but without the provision of a proof of dispersal (i.e., retrievability, only offering proof of validity). 
% The total bit complexity for $n$ PB-broadcasts from distinct processes amounts to $O(n^2L)$.
% APDB \cite{Lu2020} represents an advancement of AVID, drawing inspiration from PB. 
% It sacrifices PB's validity guarantees to incorporate AVID's dissemination and retrieval properties.
% By leveraging the need to retrieve and validate a value a constant number of times in expectation, \cite{Lu2020} attains optimal $O(nL + n^2\kappa)$ expected complexity in asynchrony.
% However, this approach falls short in the worst-case scenario of a partially synchronous solution, where $n$ reconstructions would cost $\Omega(n^2L)$.
    
% \smallskip
% \noindent \textbf{Asynchronous Data Dissemination (ADD)}. 
% In ADD \cite{das2021asynchronous}, a subset of $t+1$ correct processes initially share a common $L$-sized value $v$, and the goal is to disseminate $v$ to all correct processes, despite the presence of up to $t$ Byzantine processes. The approach of \cite{das2021asynchronous} is information-theoretically secure, tolerates up to one-third malicious nodes and has a bit complexity of $O(nL + n^2\log n)$.
% (In \name, we rely on ADD in a ``closed-box'' manner; see \Cref{section:general_framework}.)


==> sections/warm_up_hash_ext.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pseudocode description of HashFin %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \medskip
% \noindent \textbf{Pseudocode description.}
% We describe the pseudocode of \hashfin (\Cref{algorithm:hash_based_add}) from the perspective of a correct process $p_i$.
% When process $p_i$ inputs a pair $(v, d)$ (line~\ref{line:input_hashfin}), $p_i$ checks if $v \neq \bot$ (line~\ref{line:check_value_hashfin}).
% If $v \neq \bot$, it is $p_i$'s responsibility to disseminate the unique value $v = v^{\star}$; recall that we assume that at least one (and potentially only one!) correct process inputs a non-$\bot$ (i.e., $v^{\star}$) value (see Module~\ref{mod:hashfin}).
% To disseminate $v^{\star}$, process $p_i$ executes the following steps: (1) $p_i$ encodes $v^{\star}$ into $n$ RS symbols $[m_1, m_2, ..., m_n]$ (line~\ref{line:encode_value_hashfin}), and (2) $p_i$ sends the $j$-th RS symbol $m_j$ to process $p_j$ via a \textsc{disperse} message (line~\ref{line:send_disperse_hashfin}).
% Importantly, each RS symbol $m_j$ is accompanied by a valid witness that proves that $m_j$ is correctly encoded (i.e., $m_j$ belongs to a collection of correctly encoded RS symbols of value $v^{\star}$).
% Once $p_i$ receives a \textsc{disperse} message with an RS symbol $m_i$ accompanied by a valid witness that proves $m_i$'s validity (line~\ref{line:received_disperse_hash_add}), $p_i$ disseminates $m_i$ via a \textsc{reconstruct} message (line~\ref{line:broadcast_reconstruct_hash_add}).
% Lastly, when $p_i$ receives $t + 1$ RS symbols (accompanied by valid witnesses) via \textsc{reconstruct} messages (line~\ref{line:received_reconstruct_hash_add}), $p_i$ decodes value $v^{\star}$ (as all received symbols correspond to $v^{\star}$) and outputs $v^{\star}$ (line~\ref{line:output_hashfin}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% (end) pseudocode description of HashFin %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%% HashFin (algorithm) %%
%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm} [h]
% \caption{\hashfin: Pseudocode (for process $p_i$)}
% \label{algorithm:hash_based_add}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Rules:}
% \State \hskip2em Any \textsc{disperse} or \textsc{reconstruct} message with an invalid witness is ignored.
% \State \hskip2em The rules at lines~\ref{line:received_disperse_hash_add} and~\ref{line:received_reconstruct_hash_add} are activated only if $p_i$ has previously invoked an $\mathsf{input}(\cdot, \cdot)$ request.
% % \State \hskip2em Process $p_i$ executes the algorithm only after it has invoked a $\mathsf{input}(\cdot)$ request.

% \medskip
% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Digest}$ $d_i \gets \bot$
% % \State \hskip2em $\mathsf{Boolean}$ $\mathit{started}_i \gets \mathit{false}$
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{reconstruct\_broadcast}_i \gets \mathit{false}$

% \medskip
% \State \textbf{upon} $\mathsf{input}(v \in \mathsf{Value} \cup \{\bot\}, d \in \mathsf{Digest})$: \label{line:input_hashfin}
% % \State \hskip2em $\mathit{started}_i \gets \mathit{true}$
% \State \hskip2em $d_i \gets d$
% \State \hskip2em \textbf{if} $v \neq \bot$: \BlueComment{if true, then $d_i = \mathsf{digest}(v)$ (see Module~\ref{mod:hashfin})} \label{line:check_value_hashfin}
% \State \hskip4em let $[m_1, m_2, ..., m_n] \gets \mathsf{RSEnc}(v, n, t + 1)$ \label{line:encode_value_hashfin}
% % \State \hskip4em let $H^* \gets \mathsf{Eval} \big( [(1, m_1), (2, m_2), ..., (n, m_n)] \big)$
% \State \hskip4em \textbf{for each} process $p_j$:
% \State \hskip6em let $\mathcal{W}_j \gets \mathsf{CreateWit}\big( d_i, (j, m_j), [(1, m_1), (2, m_2), ..., (n, m_n)] \big)$
% \State \hskip6em \textbf{send} $\langle \textsc{disperse}, d_i, (j, m_j), \mathcal{W}_j \rangle$ to process $p_j$ \label{line:send_disperse_hashfin}

% % \medskip
% % \State \textbf{upon} receiving a \textsc{reconstruct} message from $t + 1$ processes with the same Merkle root and $\mathit{started}_i = \mathit{false}$:
% % \State \hskip2em $\mathit{started}_i \gets \mathit{true}$

% \medskip
% \State \textbf{upon} receiving a $\langle \textsc{disperse}, d_i, (i, m_i), \mathcal{W}_i \rangle$ message and $\mathit{reconstruct\_broadcast}_i = \mathit{false}$: \label{line:received_disperse_hash_add}
% \State \hskip2em $\mathit{reconstruct\_broadcast}_i \gets \mathit{true}$
% \State \hskip2em \textbf{broadcast} $\langle \textsc{reconstruct}, d_i, (i, m_i), \mathcal{W}_i \rangle$ \label{line:broadcast_reconstruct_hash_add}

% \medskip
% \State \textbf{upon} receiving a $\langle \textsc{reconstruct}, d_i, \cdot, \cdot \rangle$ message from $t + 1$ processes and $\mathit{reconstruct\_broadcast}_i = \mathit{true}$: \label{line:received_reconstruct_hash_add}
% % \State \hskip2em let $\mathit{rs\_symbols} \gets$ the set of (any) $t + 1$ received RS symbols
% \State \hskip2em \textbf{trigger} $\mathsf{output}\big( \mathsf{RSDec}(t + 1, 0, \text{the received $t + 1$ RS symbols}) \big)$ \label{line:output_hashfin}

% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% HashFin algorithm (end) %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%
%% Warmup subsection %%
%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\subsection{\warmup: Solution with $O(nL + n^3\kappa)$ Bits and $O\big( (f + 1) n \big)$ Rounds} \label{subsection:warmup}

To overview the main ideas behind our \nameopt solution, we present a simple algorithm \warmup that achieves $O(nL + n^3\kappa)$ bit complexity (optimal for $L \geq n^2\kappa$) and terminates in $O\big( (f+1)n \big)$ rounds.
As is the case with \nameopt, \warmup is optimally resilient (tolerates up to $t < n / 3$ Byzantine processes).
\warmup operates in $t + 1$ \emph{views}, where each view $V \in [1, t + 1]$ has a unique leader denoted by $\mathsf{leader}(V) = p_V$.\footnote{In \warmup (and \nameopt), leaders are elected in the round-robin fashion.}
Each view $V$ internally utilizes (1) one instance $\mathcal{GC}[V]$ of the graded consensus primitive (see \Cref{subsection:preliminaries}), and (2) one instance $\mathcal{BA}[V]$ of the binary Byzantine agreement primitive (ensuring all properties of validated agreement \emph{except for} external validity).
Moreover, if all correct processes agree on $1$ from $\mathcal{BA}[V]$, view $V$ resorts to an instance $\mathcal{DD}$ of the data dissemination primitive to allow all correct processes to decide and stop.
A graphical description of a view $V \in [1, t + 1]$ can be seen in \Cref{fig:warmup_view}, which we now delve into.

\begin{figure}[ht]
   \centering
   \includegraphics[width=\textwidth]{figures/overviews-2.pdf}
   \caption{Graphical depiction of \warmup.}
   \label{fig:warmup_view}
\end{figure}


\smallskip
\noindent \textbf{Views: structure \& rationale.}
The main idea of \warmup is to ensure that all correct processes terminate in the first view with a correct leader by deciding on the leader's proposal.
To preserve agreement, \warmup additionally guarantees that all correct processes decide the same value even in a view whose leader is faulty.
Specifically, each view $V$ operates in the following four steps:
\begin{compactenum}
    \item The leader of view $V$ broadcasts its value.
    Each correct process $p_i$ computes the hash $h_i$ of the leader's value.
    If no or an invalid value is received from the leader, $p_i$ sets $h_i$ to $\bot$.

    \item Process $p_i$ proposes $h_i$ to $\mathcal{GC}[V]$, and it decides (in $2$ synchronous rounds) a pair $(H_i, G_i)$.

    \item Process $p_i$ proposes $1$ to $\mathcal{BA}[V]$ if $H_i \neq \bot$ and $G_i = 1$.
    Crucially, if the leader of view $V$ is correct, all correct processes propose $1$ to $\mathcal{BA}[V]$.
    Indeed, if the leader is correct, it sends the same valid value to all processes, thereby guaranteeing that all processes propose the same hash $H$ (where $H$ is the hash of the received value) to $\mathcal{GC}[V]$.
    Finally, the strong validity property of $\mathcal{GC}[V]$ ensures that all correct processes decide $(H \neq \bot, 1)$ from $\mathcal{GC}[V]$.

    If $H_i = \bot$ or $G_i = 0$, process $p_i$ proposes $0$ to $\mathcal{BA}[V]$.
    Due to the explanation above, this can happen \emph{only if} the leader of view $V$ is faulty.

    \item If $0$ is decided from $\mathcal{BA}[V]$, then all correct processes proceed to the next view.
    Otherwise, all processes proceed to execute data dissemination: each correct process $p_i$ inputs a value $v_i$ to the instance $\mathcal{DD}$ of the data dissemination primitive, where $v_i$ is the value whose hash is $H_i$ (decided from $\mathcal{GC}[V]$).
    Note that if $p_i$ does not know the value whose hash is $H_i$, then $p_i$ inputs $\bot$ to $\mathcal{DD}$.
    (Importantly, the structure of view $V$ ensures that at least $t+1$ correct processes input the same non-$\bot$ value to $\mathcal{D}$.)
    %(Importantly, the structure of view $V$ ensures that at least one correct process inputs a non-$\bot$ value to $\mathcal{HF}$.)
    Once correct processes output a value from $\mathcal{DD}$, they decide that value from \warmup and stop.
\end{compactenum}

\smallskip
\noindent \textbf{Ensuring agreement \& external validity.}
% We argue that all correct processes decide the same valid value from the instance $\mathcal{DD}$ of the data dissemination primitive.
Correct processes input a value (or $\bot$) to the instance $\mathcal{DD}$ of the data dissemination primitive only after they have previously decided $1$ from $\mathcal{BA}[V]$, for some view $V \in [1, V]$.
The strong validity property of $\mathcal{BA}[V]$ ensures that some correct process $p_i$ had previously proposed $1$ to $\mathcal{BA}[V]$ (otherwise, it would be impossible to decide $1$), which implies that $p_i$ had decided a hash value $H \neq \bot$ with grade $1$ from $\mathcal{GC}[V]$.
%Furthermore, the safety property of $\mathcal{GC}[V]$ ensures that some correct process $p_j$ had proposed $D$ to $\mathcal{GC}[V]$, which implies the following: (1) process $p_j$ knows the value $v$ whose digest is $D$, and (2) value $v$ is valid (as its validity is verified by process $p_j$).
Furthermore, the awareness property of $\mathcal{GC}[V]$ ensures that a set $S$ of $|S| \geq t+1$ correct processes have proposed $H$ to $\mathcal{GC}[V]$, which implies the following: (1) each process $p_j \in S$ knows the value $v$ whose hash is $H$, and (2) value $v$ is valid (as its validity is verified by process $p_j$).
Moreover, the consistency property of $\mathcal{GC}[V]$ guarantees that all correct processes decide $H$ from $\mathcal{GC}[V]$ (potentially with grade $0$).
Therefore, the structure of view $V$ guarantees that at least $t+1$ correct processes (i.e., processes in $S$) input the same value $v$ to $\mathcal{DD}$.
Moreover, no correct process inputs a non-$\bot$ value different from $v$ to $\mathcal{DD}$ (due to the collision-resistance property of the hash function).
%one process (process $p_j$) inputs value $v$ whose digest is $D$.
Thus, the assumptions required for $\mathcal{DD}$ to operate according to its specification are satisfied.
Hence, all correct processes output valid value $v$ from $\mathcal{DD}$, decide $v$ from \warmup, and stop.

\smallskip
\noindent \textbf{Ensuring termination.}
Let $V \in [1, t + 1]$ denote the first view whose leader $\mathsf{leader}(V)$ is correct.
Process $\mathsf{leader}(V)$ sends the same valid value $v$ to all processes, thereby ensuring that all correct processes propose $v$'s hash $H = \mathsf{hash}(v)$ to $\mathcal{GC}[V]$.
The strong validity property of $\mathcal{GC}[V]$ implies that all correct processes decide $(H \neq \bot, 1)$ from $\mathcal{GC}[V]$ and propose $1$ to $\mathcal{BA}[V]$.
Therefore, all correct processes decide $1$ from $\mathcal{BA}[V]$ (due to the strong validity property of $\mathcal{BA}[V]$), proceed to execute $\mathcal{DD}$, decide $v$ from \warmup and stop.

\smallskip
\noindent \textbf{Complexity.}
In each view $V$, correct processes send (1) $O(nL)$ bits if and only if the leader of $V$ is correct, (2) $O(n^2\kappa)$ bits in $\mathcal{GC}[V]$, and (3) $O(n^2)$ bits in $\mathcal{BA}[V]$.
As correct processes are guaranteed to terminate after the first view with a correct leader (see the paragraph above) and the bit complexity of $\mathcal{DD}$ is $O(nL + n^2 \log n)$, the total bit complexity of \warmup is $f \cdot \big( O(n^2\kappa) + O(n^2) \big) + \big( O(nL) + O(n^2\kappa) + O(n^2) \big) +  O(nL + n^2\log n) = O(nL + n^2(f+1)\kappa)$ (as $\log n < \kappa$).
%$ O(nL + n^3\kappa)$ (as $f \leq t \in O(n)$).\ayaz{do we write $f$ as $O(n)$ here to simplify $O(n^2(f+\log(n))\kappa)$ into $O(n^3\kappa)$?}
Similarly, each view $V$ incurs (1) $O(1)$ rounds due to $\mathcal{GC}[V]$, and (2) $O(n)$ rounds due to $\mathcal{BA}[V]$.
Thus, \warmup incurs $(f + 1) \cdot \big( O(1) + O(n) \big) = O\big( (f + 1)n \big)$ rounds. 
 
\smallskip
\noindent \textbf{Why $O\big( (f + 1)n \big)$ rounds?}
\warmup incurs $O\big( (f + 1)n \big)$ rounds as $f$ views (with faulty leaders) can be executed before reaching a view with a correct leader.
Indeed, a faulty leader of any view can ensure that all correct processes decide on $0$ from that view's binary agreement primitive, thus preventing termination in that view.
As each view incurs $\Omega(n)$ rounds due to the round complexity of the binary agreement primitive~\cite{dolev1983authenticated}, \warmup requires $O\big( (f + 1)n \big)$ rounds.\footnote{It is possible to reduce \warmup's rounds to $O\big( (f + 1)^2 \big)$ by employing an early-stopping binary agreement algorithm (such as the one proposed in~\cite{Lenzen2022}) in each view.}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% (end) Warmup subsection %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Hence, in order to achieve $O(f)$ round complexity while following a ``leader-based'' structure, one needs to get rid of the aforementioned agreement in each view.
% That is why \nameopt swaps binary agreement with the graded consensus primitive, as detailed in the next subsection.
% \jovan{Write this better}

%%%%%%%%%%%%%%%%%%%%%%
%% Warmup algorithm %%
%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm} [h]
% \caption{\warmup: Pseudocode (for process $p_i$)}
% \label{algorithm:warmup}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Value}$ $v_i \gets \bot$ \BlueComment{$p_i$'s proposal}
% \State \hskip2em $\mathsf{Map}(\mathsf{View} \to \mathsf{Value})$ $\mathit{known\_value}_i \gets \{\bot, \bot, ..., \bot\}$

% \medskip
% \State \textbf{for each} view $V \in [1, t + 1]$:

% \smallskip
% \State \hskip2em \emph{Step 1 of view $V$:}
% \State \hskip4em \textbf{if} $p_i = \mathsf{leader}(V)$:
% \State \hskip6em \textbf{broadcast} $v_i$

% \smallskip
% \State \hskip2em initialize local variable $\mathit{received}_i \in \mathsf{Digest} \cup \{\bot\}$
% \State \hskip2em $\mathit{received}_i \gets \bot$
% \State \hskip2em \textbf{if} $v_l \in \mathsf{Value}$ is received from $\mathsf{leader}(V)$ such that $\mathsf{valid}(v_l) = \mathit{true}$:
% \State \hskip4em $\mathit{received}_i \gets \mathsf{digest}(v_l)$
% \State \hskip4em $\mathit{known\_values}_i[\mathsf{digest}(v_l)] \gets v_l$ 

% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% (end) Warmup algorithm %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% original HashExt with 3 graded consensus instances per view %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \iffalse
% \begin{algorithm} [hp]
% \caption{\nameopt: Pseudocode (for process $p_i$)}
% \label{algorithm:optimal_2}
% \begin{algorithmic} [1]
% \footnotesize

% \State \textbf{Uses:}
% \State \hskip2em Graded consensus, \textbf{instances} $\mathcal{GC}_1[V]$, $\mathcal{GC}_2[V]$, $\mathcal{GC}_3[V]$, for each $V \in [1, t + 1]$  \BlueComment{bits: $O(n^2\kappa)$; rounds: $2$}
% \State \hskip2em Data dissemination, \textbf{instance} $\mathcal{DD}$ \BlueComment{bits: $O( nL + n^2 \log n )$; rounds: $2$}

% \medskip
% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Value}$ $v_i \gets p_i$'s proposal
% \State \hskip2em $\mathsf{Hash\_Value}$ $\mathit{locked}_i \gets \bot$ \BlueComment{locked hash value}
% \State \hskip2em $\mathsf{Hash\_Value}$ $\mathit{vote}_i \gets \bot$ \BlueComment{hash to be voted for}
% \State \hskip2em $\mathsf{View}$ $\mathit{committed\_view}_i \gets \bot$ \BlueComment{view in which a hash value has been committed}
% \State \hskip2em $\mathsf{Map}( \mathsf{Hash\_Value} \to \mathsf{Value})$ $\mathit{known\_values}_i \gets \{\bot, \bot, ..., \bot\}$ \BlueComment{values corresponding to hashes}
% \State \hskip2em $\mathsf{Map}( \mathsf{View} \to \mathsf{Set}(\mathsf{Hash\_Value}) )$ $\mathit{accepted}_i \gets \{\emptyset, \emptyset, ..., \emptyset \}$ \BlueComment{accepted hashes per view}

% \medskip
% \State \textbf{-- Task 1 --}
% \State \textbf{for each} view $V \in [1, t + 1]$:

% \smallskip
% % \State \hskip2em \textbf{wait for} $2\delta$ time \BlueComment{for $\mathcal{ADD}$ to (potentially) terminate}
% \State \hskip2em \textbf{if} $\mathit{committed\_view}_i \neq \bot$ and $\mathit{commited\_view}_i + 1 = V$: complete the view after $8$ synchronous rounds 

% \State \hskip2em \textbf{if} $\mathit{commited\_view}_i \neq \bot$ and $V > \mathit{committed\_view}_i + 1$: do not execute the view

% \smallskip
% \State \hskip2em \emph{Step 1 of view $V$:} \BlueComment{$2$ synchronous rounds}
% \State \hskip4em Let $(h_1 \in \mathsf{Hash\_Value} \cup \{\bot\}, g_1 \in \{0, 1\}) \gets \mathcal{GC}_1[V].\mathsf{propose}(\mathit{locked}_i)$ \label{line:propose_gc1}

% \smallskip
% \State \hskip2em \emph{Step 2 of view $V$:} \BlueComment{$1$ synchronous round}
% \State \hskip4em \textbf{if} $p_i = \mathsf{leader}(V)$:
% \State \hskip6em \textbf{if} $h_1 \neq \bot$: \BlueComment{check if a non-$\bot$ hash is decided from $\mathcal{GC}_1[V]$}
% \State \hskip8em \textbf{broadcast} $h_1$ \BlueComment{broadcast a non-$\bot$ hash decided from $\mathcal{GC}_1[V]$} \label{line:broadcast_d1}
% \State \hskip6em \textbf{else:}
% \State \hskip8em \textbf{broadcast} $v_i$ \BlueComment{broadcast the proposed value} \label{line:broadcast_vi}

% \smallskip
% \State \hskip4em Initialize local variable $\mathit{received}_i \in \mathsf{Hash\_Value} \cup \{\bot\}$
% \State \hskip4em Let $\mathit{received}_i \gets \bot$
% \State \hskip4em \textbf{if} $V - 1 \geq 1$ and $h_l \in \mathsf{Hash\_Value}$ is received from $\mathsf{leader}(V)$ such that $h_l \in \mathit{accepted}[V - 1]$:
% \State \hskip6em Let $\mathit{received}_i \gets h_l$

% \State \hskip4em \textbf{else if} $v_l \in \mathsf{Value}$ is received from $\mathsf{leader}(V)$ such that $\mathsf{valid}(v_l) = \mathit{true}$: \label{line:check_validity_received_from_leader}
% \State \hskip6em Let $\mathit{received}_i \gets \mathsf{hash}(v_l)$
% \State \hskip6em $\mathit{known\_values}_i[\mathsf{hash}(v_l)] \gets v_l$ \BlueComment{value $v_l$ whose hash is $\mathsf{hash}(v_l)$ is ``learned''}

% \smallskip 
% \State \hskip2em \emph{Step 3 of view $V$:} \BlueComment{$2$ synchronous rounds}
% \State \hskip4em Let $(h_2 \in \mathsf{Hash\_Value} \cup \{\bot\}, g_2 \in \{0, 1\}) \gets \mathcal{GC}_2[V].\mathsf{propose}(\mathit{received}_i)$

% \smallskip
% \State \hskip2em \emph{Step 4 of view $V$:} \BlueComment{$1$ synchronous round}
% \State \hskip4em \textbf{if} $h_1 \neq \bot$ and $g_1 = 1$: \BlueComment{check if a non-$\bot$ hash with grade $1$ is decided from $\mathcal{GC}_1[V]$}
% \State \hskip6em \textbf{broadcast} $\langle \textsc{support}, h_1 \rangle$ \label{line:broadcast_happy_1}

% \State \hskip4em \textbf{else if} $h_2 \neq \bot$ and $g_2 = 1$: \BlueComment{check if a non-$\bot$ hash with grade $1$ is decided from $\mathcal{GC}_2[V]$}
% \State \hskip6em \textbf{broadcast} $\langle \textsc{support}, h_2 \rangle$ \label{line:broadcast_happy_2}
% % \State \hskip4em \textbf{else:}
% % \State \hskip6em \textbf{broadcast} $\langle \mathsf{SAD} \rangle$\ayaz{is this not used anymore?}

% \smallskip
% \State \hskip4em \textcolor{blue}{ \(\triangleright\) check if a correct process has broadcast a $\mathsf{HAPPY}$ message for some hash $h$}
% \State \hskip4em \textbf{if} exists $\mathsf{Hash\_Value}$ $h$ such that a $\langle \textsc{support}, h \rangle$ message is received from $t + 1$ processes: 
% \State \hskip6em $\mathit{accepted}_i[V] \gets \mathit{accepted}_i[V] \cup \{h\}$ \BlueComment{hash $h$ is accepted for view $V$}

% \smallskip
% \State \hskip4em \textcolor{blue}{ \(\triangleright\) check if some hash $h$ is supported by at least $t + 1$ correct processes}
% \State \hskip4em \textbf{if} exists $\mathsf{Hash\_Value}$ $h$ such that a $\langle \textsc{support}, h \rangle$ message is received from $2t + 1$ processes:
% \State \hskip6em $\mathit{vote}_i \gets h$ \BlueComment{vote for $h$}
% \State \hskip4em \textbf{else:}
% \State \hskip6em $\mathit{vote}_i \gets \bot$ \BlueComment{vote for nothing}

% \smallskip
% \State \hskip2em \emph{Step 5 of view $V$:} \BlueComment{$2$ synchronous rounds}
% \State \hskip4em Let $(h_3 \in \mathsf{Hash\_Value} \cup \{\bot\}, g_3 \in \{0, 1\}) \gets \mathcal{GC}_3[V].\mathsf{propose}(\mathit{vote}_i)$

% \smallskip
% \State \hskip2em \emph{Step 6 of view $V$:} \BlueComment{$0$ synchronous round (only local computation)}
% \State \hskip4em \textbf{if} $h_3 \neq \bot$: \BlueComment{check if a non-$\bot$ hash is decided from $\mathcal{GC}_3[V]$}
% \State \hskip6em $\mathit{locked}_i \gets h_3$ \BlueComment{hash $h_3$ is locked as some correct process might have committed it}
% \State \hskip6em \textbf{if} $h_3 = 1$ and $\mathit{committed\_view}_i = \bot$: \BlueComment{check if hash $h_3$ is decided with grade $1$}
% \State \hskip8em $\mathit{committed\_view}_i \gets V$
% \State \hskip8em \textbf{invoke} $\mathcal{DD}.\mathsf{input}(\mathit{known\_values}[h_3])$ \BlueComment{\textbf{commit hash $h_3$}} \label{line:commit_hash_value}
% \State \hskip4em \textbf{else:}
% \State \hskip6em $\mathit{locked}_i \gets \bot$ \BlueComment{no hash is locked as it is impossible that any correct processes committed in $V$}

% \medskip
% \State \textbf{-- Task 2 --} \BlueComment{executed in a separate thread}
% \State \textbf{upon} $\mathcal{DD}.\mathsf{output}(v' \in \mathsf{Value})$: \label{line:upon_output_optimal_2}
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(v')$
% \State \hskip2em \textbf{wait for} view $\mathit{committed\_view}_i + 1$ to be completed \label{line:wait_for_completion}
% \State \hskip2em \textbf{trigger} $\mathsf{stop}$ \BlueComment{process $p_i$ stops} \label{line:halt_optimal_2}

% \end{algorithmic}
% \end{algorithm}
% \fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% (end) original HashExt with 3 graded consensus instances per view %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \medskip
% \noindent \textbf{Pseudocode description.}
% \nameopt's pseudocode contains two independent (run in separate threads) tasks.
% The first task of \nameopt runs in (up to) $t + 1$ \emph{views}, where each view $V \in [1, t + 1]$ has its unique leader $\mathsf{leader}(V) = p_V$.
% Each view has 6 steps (where each step might contain multiple synchronous rounds).
% We discuss each of the steps of a view $V \in [1, t + 1]$ from the perspective of a correct process $p_i$:
% \begin{compactitem}
%     \item \emph{Step 1:}
%     In the first step of $V$, process $p_i$ proposes a digest $\mathit{lastd}_i$ to $\mathcal{GC}_1[V]$ (line~\ref{line:propose_gc1}); the digest $\mathit{lastd}_i$ is obtained in the last step of the previous view (if $V > 1$).
%     Let $p_i$ decide a pair $(d_1, g_1)$ from $\mathcal{GC}_1[V]$.

%     \item \emph{Step 2:}
%     In the second step of $V$, the leader of $V$ broadcasts either (1) a digest it obtained from $\mathcal{GC}_1[V]$ (line~\ref{line:broadcast_d1}) if the digest is non-$\bot$, or (2) its proposal (line~\ref{line:broadcast_vi}) otherwise.
%     Process $p_i$ initializes its local variable $\mathit{received}_i$ to capture information received from the leader of $V$.
%     We distinguish three cases:
%     \begin{compactitem}
%         \item Let $p_i$ receive a digest $d_l$ from the leader.
%         In this case, $p_i$ updates its $\mathit{received}_i$ variable to $d_l$ \emph{only if} $p_i$ accepted $d_l$ in the previous view (if $V > 1$).
%         If $p_i$ accepted $d_l$ in the previous view, that implies that $d_l$ was supported by at least one correct process in view $V - 1$.
%         Importantly, this means that the digest $d_l$ is a digest of a valid value that is known to at least one correct process.
%         (See the rest of the description for the clarification.)

%         \item Let $p_i$ receive a value $v_l$ from the leader.
%         In this case, $p_i$ updates its $\mathit{received}_i$ variable to the digest of $v_l$ \emph{only if} $v_l$ is valid.
%         This is crucial as it guarantees that correct processes consider only digest of valid values.

%         \item Let $p_i$ not receive anything from the leader.
%         In this case, $p_i$'s variable $\mathit{received}_i$ remains $\bot$.
%     \end{compactitem}

%     \item \emph{Step 3:}
%     Process $p_i$ proposes $\mathit{received}_i$ to $\mathcal{GC}_2[V]$ and it decides a pair $(d_2, g_2)$.

%     \item \emph{Step 4:}
%     In this step, process $p_i$ chooses whether it deems the current view as ``successful''.
%     Namely, if $p_i$ has decided a non-$\bot$ digest $d_1$ with grade $1$ from $\mathcal{GC}_1[V]$ (Step 1), $p_i$ broadcasts a $\langle \mathsf{HAPPY}, d_1 \rangle$ message.
%     Otherwise, if $p_i$ has decided a non-$\bot$ digest $d_2$ with grade $1$ from $\mathcal{GC}_2[V]$, then $p_i$ broadcasts a $\langle \mathsf{HAPPY}, d_2 \rangle$ message.
%     Otherwise, process $p_i$ broadcasts a $\langle \mathsf{SAD} \rangle$.

%     Process $p_i$ then checks if it has received some digest $d$ in at least $t + 1$ \textsc{happy} messages.
%     If so, process $p_i$ accepts $d$ in the current view $V$.
%     Note that if $p_i$ accepts $d$, that means that $d$ is the digest of a valid value.

%     Moreover, if $p_i$ receives some digest $d$ from at least $2t + 1$ $\mathsf{HAPPY}$ messages, $p_i$ updates its $\mathit{currd}_i$ variable to $d$.
%     Note that if $p_i$ updates its $\mathit{currd}_i$ variable to $d$, then every correct process accepts $d$ in the view $V$.

% \end{compactitem}



% \begin{theorem}
% \nameopt (\Cref{algorithm:optimal_2}) is correct, i.e., it satisfies agreement, external validity\footnote{Let us note that strong validity can be trivially achieved by running a second agreement algorithm $\mathcal{A}_2$ with strong validity only (e.g., \cite{Chen2021} atop \cite{Lenzen2022}) in parallel, and decide the value of (i) \nameopt if $\mathcal{A}_2$ returned $\bot$, and (ii) $\mathcal{A}_2$ otherwise.} and termination. Moreover, it achieves $O(\delta(f+1))$ latency and $O(nL + n^2 (f + 1) \kappa)$ bit complexity.
% \end{theorem}
% \begin{proof}
%     The formal proof is relegated to \Cref{section:nameopt_proof}. 
% \end{proof}
